Integrating Homomorphic Encryption and Trusted Execution Technology for Autonomous and Confidential Model Refining in Cloud

With the popularity of cloud computing and machine learning, it has been a trend to outsource machine learning processes (including model training and model-based inference) to cloud. By the outsourcing, other than utilizing the extensive and scalable resource offered by the cloud service provider, it will also be attractive to users if the cloud servers can manage the machine learning processes autonomously on behalf of the users. Such a feature will be especially salient when the machine learning is expected to be a long-term continuous process and the users are not always available to participate. Due to security and privacy concerns, it is also desired that the autonomous learning preserves the confidentiality of users' data and models involved. Hence, in this paper, we aim to design a scheme that enables autonomous and confidential model refining in cloud. Homomorphic encryption and trusted execution environment technology can protect confidentiality for autonomous computation, but each of them has their limitations respectively and they are complementary to each other. Therefore, we further propose to integrate these two techniques in the design of the model refining scheme. Through implementation and experiments, we evaluate the feasibility of our proposed scheme. The results indicate that, with our proposed scheme the cloud server can autonomously refine an encrypted model with newly provided encrypted training data to continuously improve its accuracy. Though the efficiency is still significantly lower than the baseline scheme that refines plaintext-model with plaintext-data, we expect that it can be improved by fully utilizing the higher level of parallelism and the computational power of GPU at the cloud server.

==> backprop.tex <==
\section{Backward Propagation}
\label{sec:backprop}


For each layer $l$,
let $\nabla\tilde{C}^{(l)}_i$ for $i\in\{0,\cdots,\iota_l-1\}$
denote the $i$-th ciphertext for the gradient of input, and
$\nabla\tilde{C}^{(l+1)}_i$ for $i\in\{0,\cdots,o_l-1\}$
denote the $i$-th ciphertext for the gradient of output.



\subsection{Final Layer}



\subsection{Backward Propagation: Fully-connected Layer $l$}

The design of backward propagation is mainly driven by the following goals:
\begin{itemize}
    \item 
    The workload at the TEE is minimized even at the cost of (reasonably) increasing the cost at the untrusted server. 
    \item 
    The workload at the untrusted server should be lowered and paralleled as much as possible.   
\end{itemize}
%
Here, we also consider two types of fully-connected layers the same as the above. 
However, in contrary to the forward propagation, 
we describe these types based on how many sets of outputs are encoded per ciphertext.

\subsubsection{Type I: Single Set of Outputs per Ciphertext}

This type corresponds to Type I presented in Section~\ref{sec:forward-full-1}.

\paragraph{Backward Propagation}

The backward propagation algorithm is formally presented in
Algorithm~\ref{alg:bwd-full-layer-I}.

% \begin{algorithm}[htb]
% \caption{Backward Prop. through Fully-connected Layer $l$ (Type I)}
% \label{alg:bwd-full-layer-I}

% \begin{algorithmic}[1]
% \For{$i\in\{0,\cdots,\iota'_l-1\}$}
%     \State $\nabla\tilde{C}^{(l)}_i\leftarrow 0$
%     \For{$j\in\{0,\cdots,o_l-1\}$}     
%         \State $\nabla\tilde{C}^{(l)}_i = \nabla\tilde{C}^{(l+1)}_{j}\bigodot\tilde{M}^{(l)}_{j,i}$
%     \EndFor
% \EndFor
% \end{algorithmic}
% \end{algorithm}



\paragraph{Weight Update}

Weight updating goes through the following steps:
\begin{itemize}
    \item 
    Step 1 - The gradient for each $\tilde{M}^{(l)}_{i,j}$, 
    denoted as $\nabla\tilde{M}^{(l)}_{i,j}$, is computed as $\nabla\tilde{C}^{(l+1)}_i\bigodot\tilde{C}^{(l)}_j$.
    \item 
    Step 2 - For each $\nabla\tilde{M}^{(l)}_{i,j}$, 
    where $i\in\{0,\cdots,o_l-1\}$ and $j\in\{0,\cdots,\iota'_l-1\}$,
    the elements of each n-element set is added up to the element of index $i\cdot\iota'_l+j$;
    then it is multiplied with the vector that encodes $0$'s and $1$'s where
    1 only appears at each position $p$ such that $p~\mod~n~=~i\cdot\iota'_l+j$. 
    \item 
    Step 3 - The ciphertexts resulted from the above step are split into $n$-element groups.
    \item 
    Step 4 - The ciphertexts in the same group are added up (merged such that non-zero elements are only added with zeros).
    \item 
    Step 5 - The ciphertexts resulted from the above step are decrypted by the TEE and then re-encrypted.
    \item 
    Step 6 - Each of the ciphertexts resulted from the above are split into $n$ ciphertexts (reverse of Step 4). 
    \item 
    Step 7 - For each of the ciphertexts resulted from the above,
    the non-zero element at each $n$-element set is populated (duplicated) to all the positions of the set.
    \item 
    Step 8 - Each of the ciphertexts from the above step is added to the current weight ciphertext, respectively,
    to obtain the updated weight ciphertexts. 
\end{itemize}
Note that, the TEE is involved only in step 5. 



\subsubsection{Type II: Multiple Set of Outputs per Ciphertext}

\paragraph{Backward Propagation}
Algorithm~\ref{alg:bwd-full-layer-II} formally presents the algorithm for computing the gradients of input
from the gradients of output through backward propagation at layer $l$.

\begin{algorithm}[htb]
\caption{Backward Prop. through Fully-connected Layer $l$ (Type II)}
\label{alg:bwd-full-layer-II}
\begin{algorithmic}[1]
\For{$i\in\{0,\cdots,\iota_l-1\}$}
    \State $\nabla\tilde{C}^{(l)}_i\leftarrow 0$ 
    \For{$j\in\{0,\cdots,\lceil\frac{o_l\cdot n}{s}\rceil-1\}$}     
        \State $\nabla\tilde{C}^{(l)}_i += \nabla\tilde{C}^{(l+1)}_j\bigodot\tilde{M}^{(l)}_{j,i}$
    \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}


\paragraph{Weight Update}
(similar to the Type I) 




\subsection{Background Propagation: Pooling Layer $l$}



\subsection{Background Propagation: Convolutional Layer $l$}


\paragraph{Backward Propagation}
The backward propagation algorithm is formally presented in Algorithm~\ref{alg:bwd-conv-layer}.

\begin{algorithm}[htb]
\caption{Backward Prop. through Convolutional Layer $l$}
\label{alg:bwd-conv-layer}

\begin{algorithmic}[1]

\For{$i\in\{0,\cdots,\alpha-1\}$} \Comment{each channel $i$}
    \For{$j\in\{0,\cdots,\iota_l\}$} \Comment{each input matrix $j$}
        % \For{$k\in\{0,\cdots,f_l-1\}$} \Comment{each filter matrix $k$}
        \For{$u\in\{0,\cdots,\tilde{\gamma}_{l+1}-1\}$}
            \For{$v\in\{0,\cdots,\tilde{\gamma}_{l+1}-1\}$} 
                \For{$x\in\{0,\cdots,\gamma_l-1\}$}
                    \For{$y\in\{0,\cdots,\gamma_l-1\}$}
                        \State $u'\leftarrow u\cdot\delta_l)$
                        \State $v'\leftarrow v\cdot\delta_l$
                        \State $\nabla\tilde{C}^{(l,j)}_{i,u+x,v+y} \leftarrow 0$
                        \For{$k\in\{0,\cdots,f_l-1\}$} \Comment{each filter matrix $k$}
                            \State $\nabla\tilde{C}^{(l,j)}_{i,u+x,v+y} += \nabla\tilde{C}^{(l+1,j\cdot f_l+k)}_{i,u',v'}\bigodot\hat{F}^{(l,k)}_{i,x,y}$
                        \EndFor
                    \EndFor
                \EndFor
            \EndFor
        \EndFor
    \EndFor
\EndFor

\end{algorithmic}
\end{algorithm}

\paragraph{Weight Update}
Weight updating goes through the following steps:
\begin{itemize}
    \item 
    Algorithm~\ref{alg:weight-gradient-conv-layer} is applied to compute the weight gradients.
    \item 
    For the set of $\nabla\tilde{F}^{(l,k)}_{i,x,y}$ where $k\in\{0,\cdots,f_l-1\}$, 
    channel $i\in\{0,\cdots,\alpha-1\}$,
    and $x,y\in\{0,\cdots,\gamma_l-1\}$, 
    the afore-described weight update procedure is applied to 
    update the filters with the minimal facilitation from the TEE. 
\end{itemize}

\begin{algorithm}[htb]
\caption{Computing Weight Gradients for Convolutional Layer $l$}
\label{alg:weight-gradient-conv-layer}

\begin{algorithmic}[1]

\For{$i\in\{0,\cdots,\alpha-1\}$} \Comment{each channel $i$}
    \For{$j\in\{0,\cdots,\iota_l\}$} \Comment{each input matrix $j$}
        \For{$k\in\{0,\cdots,f_l-1\}$} \Comment{each filter matrix $k$}
            \For{$x\in\{0,\cdots,\gamma_l-1\}$}
                \For{$y\in\{0,\cdots,\gamma_l-1\}$}
                    \State $\nabla\tilde{F}^{(l,k)}_{i,x,y}\leftarrow 0$
                    \For{$u\in\{0,\cdots,\tilde{\gamma}_{l+1}-1\}$}
                        \For{$v\in\{0,\cdots,\tilde{\gamma}_{l+1}-1\}$}
                        \State $u'\leftarrow u\cdot\delta_l$
                        \State $v'\leftarrow v\cdot\delta_l$
                        \State $\nabla\tilde{F}^{(l,k)}_{i,x,y} += \nabla\tilde{C}^{(l+1,j\cdot f_l+k)}_{i,u,v}\bigodot\tilde{C}^{(l,j)}_{i,u'+x,v'+y}$
                        \EndFor
                    \EndFor
                \EndFor
            \EndFor
        \EndFor
    \EndFor
\EndFor

\end{algorithmic}
\end{algorithm}










==> eval.tex <==

\section{Evaluation}
\label{sec:eval}

We implement the LHE-based inference scheme 
% (along with cross-channel and cross-filter optimizations) 
and run it on a moderate platform, i.e., a computer with Intel 2.6 GHz CPU that runs Ubuntu 20.04, 
for performance evaluation. 


% \comment{
% In this section, we aim to evaluate the performance of our proposed schemes
% (i.e., the schemes that support generic CNN model configuration with or without the cross-channel/cross-filter optimizations),
% identify the factors that affect the performance, and 
% compare our scheme to two most related schemes~\cite{gilad2016cryptonets} and~\cite{jiang2018secure}.
% Specifically, we measure the following performance metrics:
% \begin{itemize}
%     \item 
%     The computational cost for the client who outsources a CNN model to prepare (i.e., pack and encrypt) the model parameters and 
%     the communication cost for sending the encrypted model to the cloud server. Here, the computational cost is measured
%     in terms of the number of FHE encryption operations and the time spent for such operations; 
%     the communication cost is measured in terms of the number and total sizes of ciphertexts that should be sent to the server.
%     \item 
%     The computational and communication costs for the client who outsources the data to prepare (i.e., pack and encrypt) the data and send the encrypted data to the server. 
%     The costs are measured in the same way as above.
%     \item 
%     The computational cost for the server to perform the computation (i.e., forward propagation) as requested by the client. 
%     The cost is measured in terms of the numbers of FHE operations including homomorphic multiplications, rotations and additions. 
%     It is also measured as the time spent for the whole computation procedure as well as for propagation through each layer of the model. 
% \end{itemize}
% The metrics are measured when the following conditions vary:
% \begin{itemize}
%     \item 
%     the architecture of the CNN model including the number of layers, the input/output sizes and other parameters of each layer, etc.;
%     \item 
%     the number of inputs that the client requests to process in parallel;
%     \item 
%     the total number of inputs that the client requests to process.
% \end{itemize}
% We are interested in measuring the above performance metrics both as the values for certain input batches of certain given sizes and the amortized values. 
% In practice, the values for certain input batches usually indicate the latency experienced 
% by the client who submit the inputs and wait for the result; 
% the amortized values usually indicate the throughput of the system and 
% the averaged cost of the system in the long run. 

% The two compared schemes are CryptoNet~\cite{} and the scheme proposed by Jiang et al.~\cite{}.
% CryptoNet is optimized for the ideal scenarios where a large number of inputs are available at a time for massive-scale SIMD processing
% and thus the large number of slots in each ciphertext can be fully utilized. 
% Such conditions, however, are not always realistic, especially when the neural network has many layers which leads to 
% larger ciphertext size and hence larger number of slots available at each ciphertext.
% The scheme proposed by Jiang et al. is optimized for the setting of single convolutional layer and 
% hence is not applicable to generic neural network models. 
% With generic data packing and packing-aware data processing strategies, 
% our proposed scheme is able to work with any arbitrary number of inputs available at time for SIMD processing. 
% When comparing to CryptoNet, we focus on demonstrating the flexibility of scheme and 
% studying the performance implications which are mainly demonstrated by the tradeoffs between 
% instance values and amortized values of the performance metrics under varying conditions. 
% }

\subsection{CNN Models and LHE Parameters}
\label{subsec::cnn-strucutres}

% System performance is evaluated on 
We use the CNN models described in Section~\ref{subsec:cnn-model} 
with $c\in\{1,2,3,4\}$ and 
$f\in\{1,2\}$.
% ; recall that the square function is used as activation function.
%
In the following, 
we use {\it CNN c-f} (e.g., {\it CNN 2-1}) to denote a CNN model 
with $c$ convolutional layers (CLs) and $f$ fully-connected layers (FLs). 
%
% we consider CNN structures with different levels of convolutional layers (CLs) and fully connected layers (FLs) to show the effectiveness of our model. 
% As CLs and FLs are linear computation, it can be easily computed with the FHE with the addition, multiplication and rotate operations. 
% For non-linear layers like activation functions, we follow the methods in~\cite{jiang2018secure} and~\cite{gilad2016cryptonets} 
% to adopt the square activation function to approximate the results.
% Specifically, we consider CNNs with the number of CLs $i\in\{1,2,3,4\}$ and the number of FLs $j\in\{1,2\}$. %
% The different CNN structures and filter parameters are presented as follows and 
% particularly every CL followed by a square activation function in all CNN settings which are skipped in the following description. 
All experiments use the MNIST dataset~\cite{lecun1998mnist} to 
classify the ten handwritten digits and each input image of $28\times28$.
%
% Particularly, we evaluate with models:
% % \begin{itemize}
% %     \item 
%     \textcircled{1} CNN 1-2 ($c=1,f=2$), which follows the same structure as in \cite{gilad2016cryptonets,jiang2018secure}.
%     The only CL has filter parameters (4,7,3), i.e., 
%     4 filters each of side 7 per channel and stride being 3. 
%     % The weight matrices of the FLs have dimensions of $256\times64$ and $64\times10$, respectively. 
%     % \item 
%     \textcircled{2} CNN 2-1 ($c=2,f=1$), where the two CLs have filter parameters (16,7,2) and (4,5,2),
%     and the FL's weight matrix is of $64\times10$.
%     % \item 
%     \textcircled{3} CNN 2-2 ($c=f=2$), where the two CLs have filter parameters (16,7,2) and (4,5,2), 
%     and the weight matrices of the two FLs are of $64\times64$ and $64\times10$ respectively.
%     % \item 
%     \textcircled{4} CNN 3-1 ($c=3,f=1$), where the three CLs has parameters (16,3,2), (4,3,2) and (16,3,1) respective,
%     and the weight matrix of the FL is of $256\times10$.
%     % \item 
%     \textcircled{5} CNN 3-2 ($c=3,f=2$), where the three CLs have parameters (16,3,2), (4,3,2) and (16,3,1),
%     and the weight matrices of the two FLs are of $256\times64$ and $64\times10$.
%     % \item 
%     \textcircled{6} CNN 4-1 ($c=4,f=1$), where the four CLs have parameters (16,5,2), (4,3,1), (16,3,2) and (4,3,1),
%     and the weight matrix of the FL is of $16\times10$.
%     % \item 
%     \textcircled{7} CNN 4-2 ($c=4,f=2$), where the four CLs have parameters (16,5,2), (4,3,1), (16,3,2) and (4,3,1),
%     and the weight matrices of the two FLs are of $16\times64$ and $64\times10$.
% \end{itemize}
% when $c=1$ and $f=2$ (also denoted as CNN 1-2), we adopt the same structure 
% % \paragraph{CNN 1-2} in this setting, one CL and two FLs are considered which share the same structure 
% as in~\cite{gilad2016cryptonets} and~\cite{jiang2018secure}. 
% For the only CL, the filter parameters are $(4,7,3)$, i.e., 
% there are $4$ filters each of side $7$ per layer and the stride is $3$. 
% % The first FL weight matrix has dimension $256\times64$ and the second FL weight matrix has dimension $64\times10$.
% The weight matrices of the FLs have dimensions of $256\times64$ and $64\times10$, respectively. 
% Specifically, a square activation function is applied after the first FL.

% \paragraph{CNN 2-1} there are two CLs and one FL in this setting. The filter parameters tuples for these two CLs are (16,7,2) and (4,5,2). The FL weight matrix has dimension $64\times10$.

% \paragraph{CNN 2-2} two CLs and two FLs are considered and these two CLs share the same parameters as in {\it CNN 2-1}. The weight matrices for two FLs are $64\times64$ and $64\times10$.

% \paragraph{CNN 3-1} the filter parameters for three CLs are (16,3,2), (4,3,2) and (16,3,1). The weight matrix for FL has dimension $256\times10$.

% \paragraph{CNN 3-2} same configurations for three CLs are shared with {\it CNN 3-1}. For these two FLs, the weight matrices are with dimension $256\times64$ and $64\times10$.
% \paragraph{CNN 4-1} there are four CLs and one FL in this case. The filter parameters for each CL are (16,5,2), (4,3,1), (16,3,2) and (4,3,1). The weight matrix for FL is of dimension $16\times10$.
% \paragraph{CNN 4-2} in this case, these four CLs have the same settings as in {\it CNN 4-2}. The settings for two FLs weight matrices are with dimension $16\times64$ and $64\times10$.

% \subsection{LHE Parameters}
% \label{subsec::fhe-params}

We employ 
CKKS~\cite{cheon2017homomorphic} of the SEAL library~\cite{sealcrypto} as the LHE scheme. 
% which implements to support approximate computations homomorphicly.
Different polynomial modulus $N$ are used to match different CNN configurations. 
Each plaintext has ${\cal S}=\frac{N}{2}$ slots encoding up to ${\cal S}$ values. 
% In our settings, 
% to be compatible with different CNN structures, 
We adopt $N=8192$ and $N=16384$ which support 
a maximal coefficient modulus bit length of 218 and 438, respectively, to 
attain a 128-bit security level~\cite{laine2017simple}. 
Since each CL or FL (including square activation) requires 
two levels of homomorphic multiplication, 
we adjust the polynomial modulus and coefficient modulus to 
make the LHE scheme to support different settings of CNNs.
The detailed parameters 
% for different CNN models introduced in~\ref{subsec::cnn-strucutres} 
are listed in Table~\ref{tab:HE-paras}.

\begin{table}[htb]
\caption{The SEAL parameters for different CNN structures}
\label{tab:HE-paras}
\resizebox{\linewidth}{!}{
$\displaystyle
\begin{tabular}{|l|l|l|l|}
\hline
CNN models   & N     & Coefficient Modulus                     & Levels \\ \hline
\textit{CNN 1-2} & 8192  & \{34,30,30,30,30,30,34\}                & 6      \\ \hline
\textit{CNN 2-1} & 8192  & \{34,30,30,30,30,30,34\}                & 6      \\ \hline
\textit{CNN 2-2} & 16384 & \{40,30,30,30,30,30,30,40\}             & 7      \\ \hline
\textit{CNN 3-1} & 16384 & \{40,30,30,30,30,30,30,30,40\}          & 8      \\ \hline
\textit{CNN 3-2} & 16384 & \{40,30,30,30,30,30,30,30,30,40\}       & 9      \\ \hline
\textit{CNN 4-1} & 16384 & \{40,30,30,30,30,30,30,30,30,30,40\}    & 10     \\ \hline
\textit{CNN 4-2} & 16384 & \{40,30,30,30,30,30,30,30,30,30,30,40\} & 11     \\ \hline
\end{tabular}
$}
\end{table}

\subsection{Evaluation Results}


% the running environment settings

% The experiments are run on Ubuntu with an Intel ... with 32 cores rated at 2.6GHz. 
% MNIST dataset is used as the inputs for all different experiment settings and each input has dimension $28\times28$.
% For the evaluation process, we first evaluate how the number of parallel inputs and total inputs affect the performance of our model.
% Then we compare the experiments results with CryptoNets and E2DM using the same CNN architecture. 
% CNNs of different complexities are also considered and the results are reported in the following parts.

% The values in each cell reported in the following tables is either represented as a single number or a tuple with multiple values. 
% For the tuples which compose of at most four elements, it represents the number of FHE operations in the order of addition (Add), ciphertext-ciphertext multiplication (Mul), rotation (Rot) and plaintext-ciphertext (PMul) operations. The cell with 2-tuples, 3-tuples and 4-tuples match the first 2, 3 and 4 operations in the aforementioned order correspondingly.
% For our model, we describe it with pair $(n, r)$ where $n$ is the number of parallel inputs and $r$ is the number of packed ratio.

\subsubsection{Computation Time of LHE Operations} 

We first measure the computation time of 
$\oplus$, $\otimes$, {\it Rot} and {\it CMul} 
with $N=16384$ and various encryption levels. 
The results (averaged over 5000 measurements) 
are presented in Table~\ref{tab:FHE-operations}. 
% The results are recorded as the average computation time running each operation for 5000 times.
As we can see, 
$\otimes$ has the highest cost,
followed by $Rot$ whose cost is around 80\% of $\otimes$,
followed by $CMul$ whose cost is about 15-20\% of $\otimes$,
and $\oplus$ has the lowest cost. 
With the level increases, the costs for $\otimes$, $Rot$ and $CMul$ all increase linearly. 

% when the level is 6, 
% the cost for $\otimes$ is around 5 times as that of {\it CMul}, and 
% the the cost for {\it Rot} is slightly smaller than that of $\otimes$.
% Also, as the level increases,
% the costs for every operation is significantly increased. 
% When the level is 11, 
% the cost for each operation is much greater than the case of level number 6.  

\begin{table}[htb]
\centering
\caption{Execution time ($\mu s$) of LHE operations ($N=16384$)}
\label{tab:FHE-operations}
\resizebox{0.6\linewidth}{!}{
\begin{tabular}{|l|l|l|l|l|}
\hline
%                  & Add      & Mul           & Rot           & PMul \\ \hline
% \textit{CNN 1-2} & 126      & 11980         & 9279          & 2368 \\ \hline
% \textit{CNN 4-2} & 466      & 66271         & 54557         & 9507     \\ \hline
Level & $\oplus$ & $\otimes$ & \textit{Rot} & \textit{CMul} \\ \hline
2      & 93       & 6434      & 4542         & 1645          \\ \hline
3      & 127      & 10106     & 7311         & 2467          \\ \hline
4      & 172      & 14466     & 10719        & 3273          \\ \hline
5      & 209      & 19757     & 14995        & 4137          \\ \hline
6      & 253      & 25931     & 20057        & 5018          \\ \hline
7      & 298      & 33139     & 25916        & 5935          \\ \hline
8      & 345      & 39953     & 31722        & 6741          \\ \hline
9      & 397      & 49835     & 40167        & 7942          \\ \hline
10     & 443      & 57791     & 47144        & 8731          \\ \hline
11     & 498      & 68374     & 56366        & 9895          \\ \hline
\end{tabular}
}
\end{table}

\subsubsection{Scalability with Varying $n$ (number of simultaneously-available inputs)} 

We experiment with CNN 3-2 model to evaluate 
the impact of $n\in\{16,32,64,128,256,512\}$.
The cross-channel or the cross-filter optimizations are applied whenever possible
and the packing parameter $r$ is computed according to the afore-described design.
% then the number of packed ratio in the cross-filter and cross-channel optimization $r\in\{32,16,8,4,2,1\}$ correspondingly since the slots number $s=8192$ and the encoded input matrix has side $\tilde{\beta}_0=4$. 
% For the CLs, we apply the cross-filters and cross-filters alternatively to fully utilize the slots.

\begin{table*}[htb]
\centering
\caption{Computation Time for {\it CNN 3-2} (unit: second)}
\label{tab:parallel-images-delay}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
($n$, $r$)                      & Inputs        & Filters       & Weights       & CL1           & Square        & CL2           & Square        & CL3           & Square        & FL1           & FL2           &\textbf{Total}       & \textbf{Amortized}\\ \hline
(\textbf{16},32)                         & 8.076         & 2.967         & 4.668         & 22.535        & 2.013         & 15.008        & 0.916         & 0.920         & 0.018         & 3.560         & 0.704         & \textbf{45.674}               & \textbf{2.855} \\ \hline
(\textbf{32},16)                         &8.108          & 2.974         & 4.683         & 21.829        &1.943          & 13.780        & 0.886         & 0.927         & 0.018         & 3.236         & 0.692         & \textbf{43.311}               & \textbf{1.353}\\ \hline
(\textbf{64},8)                          &8.464          &6.188          &7.297          &44.310         &4.022          &24.790         &0.912          &1.740          &0.032          &3.835          &0.713          & \textbf{80.354}               & \textbf{1.256}\\ \hline
(\textbf{128},4)                         &8.409          &12.347         &12.170         &88.434         &8.074          &47.035         &0.880          &3.261          &0.058          &5.110          &0.690          & \textbf{153.542}              & \textbf{1.2}\\ \hline
(\textbf{256},2)                         &8.769          &25.088         &22.355         &177.42         &16.026         &91.092         &0.911          &6.676          &0.118          &8.65           &0.707          & \textbf{301.598}              & \textbf{1.178}\\ \hline
(\textbf{512},1)                         &8.742          &48.978         &41.712         &344.842        &32.435         &179.136        &0.885          &12.971         &0.224          &15.145         &0.696          & \textbf{586.334}              & \textbf{1.145}\\ \hline
\end{tabular}
}
\end{table*}

\begin{table}[htb]
\centering
\caption{Numbers of LHE operations at every stages of {\it CNN 1-2}. Input size: 4096 for CryptoNets; 64 for E2DM and our scheme. 
Each single value in inputs and parameters encryption represent the number of encryption times and each value in Square row represents the number of ciphertext-ciphertext multiplication operations. \textbf{The tuples represent the number of LHE operations in the order of $\oplus$, $\otimes$, $Rot$ and $CMult$. 
The 2-tuples, 3-tuples and 4-tuples match the first 2, 3 and 4 operations respectively.}
}
\label{tab:cnn-1-2-times}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|l|l|l|}
\hline
                      & Our Scheme        & E2DM                      & CryptoNets    \\ \hline
LHE Level             & 6                 & 8                        & 6           \\ \hline
Enc. Inputs         & 49                & 49                        & 784           \\ \hline
Enc. Filter         & 196               & 196                       & 196           \\ \hline %\cline{2-5} 
Enc. Weight1        & 256               & 4                         & 16384         \\ \hline %\cline{2-5} 
Enc. Weight2        & 64                & 1                         & 640           \\ \hline
Preprocess Weight1     &                   &  (1024,0,608,768)         &          \\ \hline %\cline{2-5} 
Preprocess Weight2     &                   &  (138,0,44,148)          &          \\ \hline
CL1                    & (192,196,0)       & (192,196,0)               & (12288,12544) \\ \hline %\cline{2-5} 
Square                 & 4                 & 4                         & 256           \\ \hline %\cline{2-5} 
FL1                    & (576,256,384)     & (512,256,320,256)         & (16320,16384) \\ \hline %\cline{2-5} 
Square                 & 64                & 1                         & 64            \\ \hline %\cline{2-5} 
FL2                    & (63,64,0)         & (77,10,29,64)            & (630,640)     \\ \hline %\cline{2-5} 
\textbf{Total}         & (831,584,384)     & (781,467,349,320)         & (29238,29888)     \\ \hline %\cline{2-5} 
\textbf{Amortized}     & (13,9.1,6)     & (12.2,7.3,5.5,5)         & (7.1,7.3)     \\ \hline
\end{tabular}

% \begin{tabular}{|l|l|l|l|}
% \hline
%                       & Our Scheme        & E2DM                      & CryptoNets    \\ \hline
% LHE Level             & 6                 & 8                        & 6           \\ \hline
% Enc. Inputs         & 49                & 49                        & 784           \\ \hline
% Enc. Filter         & 196               & 196                       & 196           \\ \hline %\cline{2-5} 
% Enc. Weight1        & 256               & 4                         & 16384         \\ \hline %\cline{2-5} 
% Enc. Weight2        & 64                & 1                         & 640           \\ \hline
% Preprocess Weight1     &                   &  (0,608)         &          \\ \hline %\cline{2-5} 
% Preprocess Weight2     &                   &  (0,44)          &          \\ \hline
% CL1                    & (196,0)       & (196,0)               & (12544,0) \\ \hline %\cline{2-5} 
% Square                 & 4                 & 4                         & 256           \\ \hline %\cline{2-5} 
% FL1                    & (256,384)     & (256,320)         & (16384,0) \\ \hline %\cline{2-5} 
% Square                 & 64                & 1                         & 64            \\ \hline %\cline{2-5} 
% FL2                    & (64,0)         & (10,29)            & (640,0)     \\ \hline %\cline{2-5} 
% \textbf{Total}         & (584,384)     & (467,349)         & (29888,0)     \\ \hline %\cline{2-5} 
% \textbf{Amortized}     & (9.1,6)     & (7.3,5.5)         & (7.3,0)     \\ \hline
% \end{tabular}

}
\end{table}


Table~\ref{tab:parallel-images-delay} presents the computation time for 
encoding/encrypting initial input data and model parameters (in the columns labelled {\em Inputs}, {\em Filters} and {\em Weights}),
and propagating through the layers (in the columns labelled {\em CL1-3}, {\em FL1-2}, and {\em Square} for activation function).
The table also shows the total time for each forward propagation round (in the column labelled {\em Total})
and the averaged time for each input image (in the column labelled {\em Amortized}). 
As we can see,
the total time increases with $n$ while 
the amortized time (i.e., the average time for processing each input image) decreases. 
This demonstrates the following trade-off: 
the smaller is the scale of simultaneously-available input, 
the shorter is the delay for obtaining the inference result 
(indicated by column {\em Total}) and 
the lower is the system throughput (indicated by column {\em Amortized}) 
Meanwhile, 
% we can also find that, 
the difference in amortized time is not significant when 
compared to the difference in the input size.
Specifically, as $n$ changes from $16$ to $512$, 
the amortized time changes only from $2.855s$ to $1.145s$.
This indicates that, our proposed design 
% (including the cross-channel and cross-filter optimizations)
has good {\em scalability} in terms of that 
{\em its performance increases with the size of simultaneously-available inputs
and meanwhile the performance does not degrade significantly when the input size is small}. 


% The detailed delay for each layer is presented in table~\ref{tab:parallel-images-delay}. 
% Similarly, when more inputs are processed in parallel, the less is the amortized delay.


% \comment{
% \begin{table}[htb]
% \caption{Number of $\otimes$ operations for encrypting inputs and model parameters for {\it CNN 3-2}}
% \label{tab:parallel-images-paras}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{|l|l|l|l|l|l|l|}
% \hline
% ($n$, $r$) & Inputs & Filter1 & Filter2 & Filter3 & Weight1 & Weight2 \\ \hline
% (16,32)                         & 225            & 9                     & 36                    & 36                    & 64                    & 64                    \\ \hline
% (32,16)                         & 225            & 9                     & 36                    & 36                    & 64                    & 64                    \\ \hline
% (64,8)                          & 225            & 18                    & 72                    & 72                    & 128                   & 64                    \\ \hline
% (128,4)                         & 225            & 36                    & 144                   & 144                   & 256                   & 64                    \\ \hline
% (256,2)                         & 225            & 72                    & 288                   & 288                   & 512                   & 64                    \\ \hline
% (512,1)                         & 225            & 144                   & 576                   & 576                   & 1024                  & 64                    \\ \hline
% \end{tabular}
% }
% \end{table}

% The numbers of $\otimes$ for clients to encode/encrypt inputs and model parameters are 
% presented in Table~\ref{tab:parallel-images-paras}.
% With the increase of parallel images, the number of encryption and generated ciphertexts increases with the corresponding ratio. When the parallel images number is 16, we could pack 32 filters or channels together. In the {\it CNN 3-2} setting, however, there are at most 16 filters or channels which makes the slots in case $(16,32)$ are not fully utilized and hence the operation times are the same as in case $(32,16)$. 
% }



% \comment{%save for more complete version!
% Table~\ref{tab:parallel-images-forward} shows the number of LHE operations for each CNN layer.
% The first CL and third CL apply the cross-filter optimization while the second CL uses the cross-channel optimization. 
% When the number of parallel images increase, 
% the number of addition and multiplication operations in CLs with cross-filter packing and 
% the number of multiplication operations in CL with cross-channel packing increase with the same ratio. 
% For the second CL with cross-channels packing which requires rotation operations to sum up all channel values, 
% the greater the packed ratio, the more is the rotation operations.
% For the FLs, the first FL has each output neuron as a separate ciphertext, 
% hence the more parallel images (less packed ratio), 
% the more multiplication operations and less rotation operations. 
% The second FL always have the same operations when the number of parallel images varies, 
% because the outputs with ten neurons are packed into one ciphertext and the slots are not fully filled.
% Hence, the total addition and multiplication operations in one forward propagation pass increase and 
% the number of total rotation operations decreases with the increment of $n$. 
% The number of amortized operations per input decreases when $n$ increases.

% \begin{table*}[htb]
% \centering
% \caption{The number of FHE operations in {\it CNN 3-2} forward propagation. The tuple in each CL and FL represent the number of addition, multiplication and rotation. For Square column, the values represent the number of square/multiplication operations.}
% \label{tab:parallel-images-forward}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
% \hline
% ($n$, $r$)                      & CL1           & Square & CL2              & Square & CL3         & Square & FL1             & FL2       & \textbf{Total}      & \textbf{Amortized} \\ \hline
% (16,32)                         & (392,441,0)   & 49     & (468,324,180)    & 36     & (35,36,0)   & 1      & (574,64,576)    & (63,64,0) & (1532,1015,756)     &(95.8,63.4,47.3)\\ \hline
% (32,16)                         & (392,441,0)   & 49     & (432,324,144)    & 36     & (35,36,0)   & 1      & (512,64,512)    & (63,64,0) & (1434,1015,656)                    &(44.8,31.7,20.5)\\ \hline
% (64,8)                          & (784,882,0)   & 98     & (720,648,108)    & 36     & (70,72,0)   & 2      & (512,128,448)   & (63,64,0) & (2149,1930,556)                    &(33.6,30.2,8.7)\\ \hline
% (128,4)                         & (1568,1764,0) & 196    & (1332,1296,72)   & 36     & (140,144,0) & 4      & (576,256,384)   & (63,64,0) & (3679,3760,456)                   &(28.7,29.4,3.4)\\ \hline
% (256,2)                         & (3136,3528,0) & 392    & (2592,2592,36)   & 36     & (280,280,0) & 8      & (768,512,320)   & (63,64,0) & (6839,7412,356)                    &(26.7,29,1.4) \\ \hline
% (512,1)                         & (6272,7056,0) & 784    & (5148,5184,0)    & 36     & (570,576,0) & 16     & (1216,1024,256) & (63,64,0) &  (13269,14740,256)                   &(25.9,28.9,0.5)  \\ \hline
% \end{tabular}
% }
% \end{table*}
% }



\subsubsection{Comparison with CryptoNets and E2DM}

We compare the performance of our scheme
with CryptoNets and E2DM, which are also based on LHE and the most related to our scheme. 
%
As the LHE systems employed by the compared schemes are not CKKS, which is used in our scheme,
and the reported evaluation results~\cite{jiang2018secure} for them
are obtained at different platforms, 
we do not directly compare in terms of measured computation time.
Instead, we choose to count the numbers of LHE operations that each of the schemes need to conduct when they are given the same input.
%
Also note that, E2DM supports only one convolutional layer, 
so comparison is conducted based on the CNN 1-2 model. 
%
Both E2DM and our scheme takes 64 images as parallel inputs,
while CryptoNets takes 4096 images as parallel inputs (as its best performance is attained when all the 4096 slots are used). 


Table~\ref{tab:cnn-1-2-times} shows the main comparison results among the three schemes. 
Comparing CrytoNets with the other schemes,
CrytoNets has the highest total cost due to the large input size;
in fact, even when the number of simultaneously-available inputs is smaller,
CrytoNets still needs such cost since it is not adaptive to input size. 
%
When the size of simultaneously-available inputs is 4096, it has the lowest amortized cost.
Specifically, it needs only $7.3$ $\otimes$ operations for each input images, by average,
while E2DM needs $7.3$ $\otimes$, $5.5$ $Rot$ and $5$ $CMult$ operations, and
our scheme needs $9.1$ $\otimes$ and $6$ $Rot$ operations.

\begin{table}[htb]
\centering
\caption{Number of LHE operations at different levels. }
\label{tab:cnn-1-2-levels}
\resizebox{.85\linewidth}{!}{
\begin{tabular}{|c|cccc|cccc|}
\hline
\multicolumn{1}{|l|}{} & \multicolumn{4}{c|}{Our Scheme}                                                                             & \multicolumn{4}{c|}{E2DM}                                                                                          \\ \hline
Level           & \multicolumn{1}{c|}{$\oplus$} & \multicolumn{1}{c|}{$\otimes$} & \multicolumn{1}{c|}{\textit{Rot}} & \textit{CMul} & \multicolumn{1}{c|}{$\oplus$} & \multicolumn{1}{c|}{$\otimes$} & \multicolumn{1}{c|}{\textit{Rot}} & \textit{CMul} \\ \hline
7                      & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{-}         & \multicolumn{1}{c|}{-}            & -             & \multicolumn{1}{c|}{192}      & \multicolumn{1}{c|}{196}       & \multicolumn{1}{c|}{-}            & -             \\ \hline
6                      & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{-}         & \multicolumn{1}{c|}{-}            & -             & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{4}         & \multicolumn{1}{c|}{-}            & -             \\ \hline
5                      & \multicolumn{1}{c|}{192}      & \multicolumn{1}{c|}{196}       & \multicolumn{1}{c|}{-}            & -             & \multicolumn{1}{c|}{256}      & \multicolumn{1}{c|}{-}         & \multicolumn{1}{c|}{320}          & 256           \\ \hline
4                      & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{4}         & \multicolumn{1}{c|}{-}            & -             & \multicolumn{1}{c|}{256}      & \multicolumn{1}{c|}{256}       & \multicolumn{1}{c|}{-}            & -             \\ \hline
3                      & \multicolumn{1}{c|}{576}      & \multicolumn{1}{c|}{256}       & \multicolumn{1}{c|}{384}          & -             & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{1}         & \multicolumn{1}{c|}{-}            & -             \\ \hline
2                      & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{64}        & \multicolumn{1}{c|}{-}            & -             & \multicolumn{1}{c|}{64}       & \multicolumn{1}{c|}{-}         & \multicolumn{1}{c|}{26}           & 64            \\ \hline
1                      & \multicolumn{1}{c|}{63}       & \multicolumn{1}{c|}{64}        & \multicolumn{1}{c|}{-}            & -             & \multicolumn{1}{c|}{13}       & \multicolumn{1}{c|}{10}        & \multicolumn{1}{c|}{3}            & -             \\ \hline
\end{tabular}
}
\end{table}

However, the above comparison does not indicate that E2DM is more efficient than our scheme,
because it only counts the number of LHE operations but 
does not consider the impact of encryption level. 
Table~\ref{tab:cnn-1-2-levels} shows the distribution of the LHE operations at different levels. 
As we can see, 
the LHE operations of E2DM occur at higher levels that our scheme.
Together with the level-specific LHE operation costs shown in Table~\ref{tab:FHE-operations}, 
E2DM should incur higher cost.

As we can also see from Table~\ref{tab:cnn-1-2-times}, 
both CryptoNets and our scheme demand the highest encryption level of 6, 
while the level needed by E2DM is 8;
note that, as shown by Table~\ref{tab:FHE-operations}, 
higher level implies most costly LHE operations. 
Regarding input encryption, 
E2DM and our scheme use the same packing method when 
the input size is 64 and thus have the same cost; 
CryptoNets has higher cost due to large input size.
Regarding model encryption and preprocessing, 
our scheme has higher cost in encryption than E2DM, 
but E2DM needs to preprocess weight matrices which is not needed by our scheme;
nevertheless, these are just one-time cost. 

Overall, the comparisons indicate that,
{\em our scheme is more efficient than E2DM mainly due to the smaller encryption level that we need}.
Also, {\em CrytoNets has the lowest amortized cost but this is attainable only when a large number of inputs are simultaneously available}. 




% The CNN architecture used in CryptoNets and E2DM is {\it CNN 1-2} which has one CL and two FLs and the CL and the first FL are followed by a square activation function. 
% In our experiments, we choose parallel inputs number $n$ to be 16 and 64 and polynomial modulus $N=8192$.
% Based on the filter parameters, we can get $\tilde{\beta}_0=8$.
% When $n=16$, the pack ratio $r=4$ then all slots are utilized and when $n=64$, the pack ratio $r=1$, that is the cross-filter and cross-channel optimization are not applied into the CL. 
% The delay for each layer with different settings of ($n$, $r$) is showed in table~\ref{tab:cnn-1-2-delay}.
% Based on the experiment results, we can achieve a total forward propagation delay of 2.488 seconds when $n=16$ and achieve a amortized delay of 0.069 when the number of parallel inputs is 64.

% We compare our model with CryptoNets and E2DM in the number of FHE operations. 
% The results are presented in table~\ref{tab:cnn-1-2-times}.
% Comparing Our Model-(64,1) with E2DM where both parallel 64 inputs at one forward propagation pass and share the same packing methods in one CL case, for the FL weight matrices, our model incurs higher encryption costs since the weights in E2DM are fully packed into a matrix without duplicates. 
% However, in order to compute the matrix multiplication in FLs, E2DM requires extra computations to generate the dependency matrices that is the Preprocess Matrices rows in the table. 
% And one FL computation requires a depth of 3 multiplications in E2DM because of the matrices generation while our model only requires 1 depth of multiplication. For the operations in FLs, the E2DM requires extra plaintext-ciphertext multiplications to generate the dependent matrices related to the convolutional outputs and less ciphertext-ciphertext multiplications.
% Regarding to the model efficiency, our model is comparable with E2DM based on the total and amortized operations. 
% The E2DM, however, requires a higher FHE level which in turn leads to higher computation cost when $N$ is larger from the measurement of table~\ref{tab:FHE-operations} 
% and the E2DM cannot be applied to generic CNN models with more than one CL like the {\it CNN 2-1} etc.

% When the number of available inputs is small, our model can further be optimized with cross-filter packing in CL and generate less ciphertexts as shown in the case of Our Model-(16,4). And less total operations are required in one forward propagation pass compared with E2DM.

% In CryptoNets, the number of parallel inputs $n=s=4096$ and each neuron is a separate ciphertext. 
% As for the inputs encryption, the CryptoNets require $28\times28$ encryption operations while our model requires $\tilde{\gamma}^2_0=49$ encryption operations. 
% For the model parameters encryption and forward propagation process, our model utilize the SIMD operations which achieves less FHE operations compared with CryptoNets.
% Comapred with our model and E2DM, the CryptoNets has the lowest amortized delay as it achieves the highest inputs parallelism which requires the user having a huge amount of inputs ready for processing. 
% Furthermore, the increase ratio for each stage of our model compared with CryptoNets is bound by $r\tilde{\beta}^2_0$ in CLs and bounded by $\frac{s}{n}$ in FLs.

% \paragraph{Theoretical Analysis} In our model, for each CL $i$ with cross-filter packing, the number of inputs ciphertext is $\tilde{\gamma}_i^2\times\alpha_i$ and the number of filter ciphertexts is $\alpha_i\times\gamma_i^2\times\lceil\frac{\epsilon_i}{r}\rceil$. The number of addition is $\tilde{\gamma}_{i+1}^2\times\lceil\frac{\epsilon_i}{r}\rceil\times(\alpha_i\times\gamma_i^2-1)$ and the number of multiplication is $\tilde{\gamma}_{i+1}^2\times\lceil\frac{\epsilon_i}{r}\rceil\times\alpha_i\times\gamma_i^2$.
% For each CL $i$ with cross-channel packing, the number of inputs cipheretxt is $\tilde{\gamma}_i^2\times\lceil\frac{\alpha_i}{r}\rceil$ and the number of filter ciphertexts is $\epsilon_i\times\gamma_i^2\times\lceil\frac{\alpha_i}{r}\rceil$.
% The number of addition in CL computation is $\tilde{\gamma}_{i+1}^2\times\epsilon_i\times(\lceil\frac{\alpha_i}{r}\rceil\times\gamma_i^2-1)+\tilde{\gamma}_{i+1}^2\times\epsilon_i\times log p$ and the number of multiplication is $\tilde{\gamma}_{i+1}^2\times\epsilon_i\times\lceil\frac{\alpha_i}{r}\rceil\times\gamma_i^2$.
% And the number of rotation operations is $\tilde{\gamma}_{i+1}^2\times\epsilon_i\times log p$.
% In CryptoNets, for each CL $i$, the number of inputs ciphertext is $\beta_i^2\times\alpha_i$ and the number of filter ciphertexts is $\epsilon_i\times\alpha_i\times\gamma_i^2$. The number of addition operations in CL is $\beta_{i+1}^2\times\epsilon_i\times(\alpha_i\times\gamma_i^2-1)$ and the number of multiplication operations is $\beta_{i+1}^2\times\epsilon_i\times\alpha_i\times\gamma_i^2$.
% Then for each FHE operations, the reduced ratio from CryptoNets to our model is bounded by $r\times\frac{\tilde{\gamma}_{i+1}^2}{\beta_{i+1}^2}$. Since $\tilde{\gamma}_{i}=\gamma_i+(\tilde{\gamma}_{i+1}-1)\times\delta_i$,  $\beta_{i}=\gamma_i+(\beta_{i+1}-1)\times\delta_i$, $\tilde{\gamma}_{c}=1$ and $\beta_{c}=\tilde{\beta}_0$ where $c$ is the index of the last convolutional layer, we can get that for each $j\in\{1,\cdots,c\}$, $\frac{\tilde{\gamma}_j^2}{\beta_j^2}\leq \tilde{\beta}_0^2$, hence we have $r\times\frac{\tilde{\gamma}_{i+1}^2}{\beta_{i+1}^2}\leq r\times\tilde{\beta}_0^2$ for $i\in\{0,\cdots,c-1\}$.

% For FL $i$, assume the number of input neurons is $\iota_i$ and the number of output neurons is $o_i$.
% With the {\it Type-I} packing, the number of input ciphertexts $\iota'_i$ is either $\frac{\iota_i}{\tilde{\beta}_0^2}$ or $\frac{\iota_i}{r\times\tilde{\beta}_0^2}$ corresponding to the last CL uses cross-filter and cross-channel respectively. 
% The number of ciphertexts for encrypting weights is $\iota'_i\times o_i$.
% Then the number of addition is $(\iota'_i-1)\times o_i+o_i\times log\frac{\iota_i}{\iota'_i}$, the number of multiplication is $\iota'_i\times o_i$ and the number of rotation is $o_i\times log\frac{\iota_i}{\iota'_i}$.
% With the {\it Type-II} packing, the number of input ciphertexts is $\iota_i$ and the number of output ciphertexts $o'_i$ is $\frac{o_i}{s/n}$.
% The number of ciphertexts for encrypting weights is $\iota_i\times o'_i$.
% The number of addition is $(\iota_i-1)\times o'_i$ and the number of multiplication is $\iota_i\times o'_i$.
% In CryptoNets, the weight ciphertexts are $\iota_i\times o_i$, the number of addition is $(\iota_i-1)\times o_i$ and the number of multiplication is $\iota_i\times o_i$. 
% Therefore, the number of encryptions, additions and multiplications is bounded by $\frac{s}{n}$.

% \begin{table}[htb]
% \centering
% \caption{The delay for {\it CNN 1-2} on MNIST in seconds.}
% \label{tab:cnn-1-2-delay}
% \begin{tabular}{|l||*{2}{c|}}
% \hline
% \backslashbox{\it CNN 1-2}{($n$, $r$)}
%               & Our Model-(16,4) & Our Model-(64,1) \\ \hline\hline
% Encrypt Inputs & 0.461  & 0.561  \\ \hline
% Encrypt Model  & 1.69   & 5.235  \\ \hline
% CL1            & 0.479  & 1.808  \\ \hline
% Square         & 0.007  & 0.026  \\ \hline
% FL1            & 1.579  & 2.204  \\ \hline
% Square         & 0.215  & 0.212  \\ \hline
% FL2            & 0.208  & 0.186  \\ \hline
% Total          & 2.488  & 4.436 \\ \hline
% Amortized      & 0.156  & 0.069 \\ \hline
% \end{tabular}
% \end{table}

% \begin{table*}[htb]
% \centering
% \caption{The number of FHE operations in different stages with model {\it CNN 1-2} comparing CryptoNets, E2DM and our model with ($n$, $r$) to be (16,4) and (64,1). 
% % Each single value in inputs and parameters encryption represent the number of encryption times and each value in Square row represents the number of ciphertext-ciphertext multiplication operations. The tuples represent the number of FHE operations in the order of addition, ciphertext-ciphertext multiplication, rotation and plaintext-ciphertext multiplication. The 2-tuples, 3-tuples and 4-tuples match the first 2, 3 and 4 operations respectively.
% }
% \label{tab:cnn-1-2-times}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{|l|l|l|l|l|l|}
% \hline
%                                                                         &                       & Our Model-(16,4)  & Our Model-(64,1)  & E2DM                      & CryptoNets    \\ \hline
%                                                                         &FHE Levels             & 6                 & 6                 & 10                        & 6           \\ \hline
%                                                                         &Encrypt Inputs         & 49                & 49                & 49                        & 784           \\ \hline
% \multirow{3}{*}{Encrypt Models}                                         &Encrypt Filter         & 49                & 196               & 196                       & 196           \\ \cline{2-6} 
%                                                                         &Encrypt Weight1        & 64                & 256               & 4                         & 16384         \\ \cline{2-6} 
%                                                                         &Encrypt Weight2        & 64                & 64                & 1                         & 640           \\ \hline
% \multicolumn{1}{|c|}{\multirow{2}{*}{Preprocess Weight Matrices}}       &Preprocess Weight1     &                   &                   &  (1024,0,608,768)         &          \\ \cline{2-6} 
% \multicolumn{1}{|c|}{}                                                  &Preprocess Weight2     &                   &                   &  (138,0,44,148)          &          \\ \hline
% \multirow{7}{*}{Forward Propagation}                                    &CL1                    & (48,49,0)         & (192,196,0)       & (192,196,0)               & (12288,12544) \\ \cline{2-6} 
%                                                                         &Square                 & 1                 & 4                 & 4                         & 256           \\ \cline{2-6} 
%                                                                         &FL1                    & (512,64,512)      & (576,256,384)     & (512,256,320,256)         & (16320,16384) \\ \cline{2-6} 
%                                                                         &Square                 & 64                & 64                & 1                         & 64            \\ \cline{2-6} 
%                                                                         &FL2                    & (63,64,0)         & (63,64,0)         & (77,10,29,64)            & (630,640)     \\ \cline{2-6} 
%                                                                         &\textbf{Total}         & (623,242,512)      & (831,584,384)     & (781,467,349,320)         & (29238,29888)     \\ \cline{2-6} 
%                                                                         &\textbf{Amortized}     & (38.9,15.1,32)      & (13,9.1,6)     & (12.2,7.3,5.5,5)         & (7.1,7.3)     \\ \hline
% \end{tabular}
% }
% \end{table*}


% % Please add the following required packages to your document preamble:
% % \usepackage[normalem]{ulem}
% % \useunder{\uline}{\ul}{}
% \begin{table}[htb]
% \centering
% \caption{The number of FHE operations at different levels. }
% \label{tab:cnn-1-2-levels}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{|c|cccc|cccc|}
% \hline
% \multicolumn{1}{|l|}{} & \multicolumn{4}{c|}{Our model-(64, 1)}                                                                             & \multicolumn{4}{c|}{E2DM}                                                                                          \\ \hline
% Level number           & \multicolumn{1}{c|}{$\oplus$} & \multicolumn{1}{c|}{$\otimes$} & \multicolumn{1}{c|}{\textit{Rot}} & \textit{CMul} & \multicolumn{1}{c|}{$\oplus$} & \multicolumn{1}{c|}{$\otimes$} & \multicolumn{1}{c|}{\textit{Rot}} & \textit{CMul} \\ \hline
% 7                      & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{-}         & \multicolumn{1}{c|}{-}            & -             & \multicolumn{1}{c|}{192}      & \multicolumn{1}{c|}{196}       & \multicolumn{1}{c|}{-}            & -             \\ \hline
% 6                      & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{-}         & \multicolumn{1}{c|}{-}            & -             & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{4}         & \multicolumn{1}{c|}{-}            & -             \\ \hline
% 5                      & \multicolumn{1}{c|}{192}      & \multicolumn{1}{c|}{196}       & \multicolumn{1}{c|}{-}            & -             & \multicolumn{1}{c|}{256}      & \multicolumn{1}{c|}{-}         & \multicolumn{1}{c|}{320}          & 256           \\ \hline
% 4                      & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{4}         & \multicolumn{1}{c|}{-}            & -             & \multicolumn{1}{c|}{256}      & \multicolumn{1}{c|}{256}       & \multicolumn{1}{c|}{-}            & -             \\ \hline
% 3                      & \multicolumn{1}{c|}{576}      & \multicolumn{1}{c|}{256}       & \multicolumn{1}{c|}{384}          & -             & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{1}         & \multicolumn{1}{c|}{-}            & -             \\ \hline
% 2                      & \multicolumn{1}{c|}{-}        & \multicolumn{1}{c|}{64}        & \multicolumn{1}{c|}{-}            & -             & \multicolumn{1}{c|}{64}       & \multicolumn{1}{c|}{-}         & \multicolumn{1}{c|}{26}           & 64            \\ \hline
% 1                      & \multicolumn{1}{c|}{63}       & \multicolumn{1}{c|}{64}        & \multicolumn{1}{c|}{-}            & -             & \multicolumn{1}{c|}{13}       & \multicolumn{1}{c|}{10}        & \multicolumn{1}{c|}{3}            & -             \\ \hline
% \end{tabular}
% }
% \end{table}



\subsubsection{Applicability to Different CNN Models}

To show the applicability of our model to generic CNN models, 
we evaluate our scheme with the CNN models whose configurations and parameters listed in section~\ref{subsec::cnn-strucutres}.
% and~\ref{subsec::fhe-params}. 
Due to space limit,
we show only the results of two settings in Tables~\ref{tab:cnn-2-1} and \ref{tab:cnn-4-2}. 
% consider different depth of CNN architectures. 
% The CNN structures and corresponding parameters are listed in section~\ref{subsec::cnn-strucutres} and~\ref{subsec::fhe-params}.

\begin{table}[htb]
\centering
\caption{LHE operations and time for {\it CNN 2-1} (Our scheme: n=16, r=16).}
\label{tab:cnn-2-1}
\resizebox{\linewidth}{!}{
% \begin{tabular}{|l|ll|l|}
% \hline
%                      & \multicolumn{2}{c|}{LHE Operations}                           & \multicolumn{1}{c|}{Time}             \\ \hline
%                      & \multicolumn{1}{l|}{Our Scheme}                  & \multicolumn{1}{l|}{CryptoNets}   & Our Scheme  \\ \hline
% Enc.  Inputs             & \multicolumn{1}{l|}{225}                      & \multicolumn{1}{l|}{784}          & 3.183   \\ \hline %\cline{2-5}
% Enc.  Filters            & \multicolumn{1}{l|}{149}                      & \multicolumn{1}{l|}{2384}         & 2.12  \\ \hline %\cline{2-7}
% Enc.  Weights            & \multicolumn{1}{l|}{40}                       & \multicolumn{1}{l|}{40}           & 0.561   \\ \hline %\cline{2-7}
%  \textbf{Total}      & \multicolumn{1}{l|}{189}                      & \multicolumn{1}{l|}{2424}         & 2.681  \\ \hline %\cline{2-7}
%   CL1                & \multicolumn{1}{l|}{(1200,1225)}              & \multicolumn{1}{l|}{(19200,19600)}& 15.882 \\ \hline %\cline{2-7}
%   Square             & \multicolumn{1}{l|}{25}                       & \multicolumn{1}{l|}{400}          & 0.251    \\ \hline %\cline{2-7}
%   CL2                & \multicolumn{1}{l|}{(112,100,16)}             & \multicolumn{1}{l|}{(1590,1600)}  & 0.859  \\ \hline %\cline{2-7}
%   Square             & \multicolumn{1}{l|}{4}                        & \multicolumn{1}{l|}{64}            & 0.021   \\ \hline %\cline{2-7}
%   FL1                & \multicolumn{1}{l|}{(110,40,80)}              & \multicolumn{1}{l|}{(630,640)}   & 0.258   \\ \hline %\cline{2-7}
%  \textbf{Total}      & \multicolumn{1}{l|}{(1422,1394,96)}           & \multicolumn{1}{l|}{(119094,123104)}     &17.271 \\ \hline %\cline{2-7}
%  \textbf{Amortized}  & \multicolumn{1}{l|}{(88.9,\textbf{87.1,6})}            & \multicolumn{1}{l|}{(29.1,\textbf{30.1})}  &1.079        \\ \hline
% \end{tabular}

\begin{tabular}{|l|ll|l|}
\hline
                     & \multicolumn{2}{c|}{LHE Operations}                           & \multicolumn{1}{c|}{Time}             \\ \hline
                     & \multicolumn{1}{l|}{Our Scheme}                  & \multicolumn{1}{l|}{CryptoNets}   & Our Scheme  \\ \hline
Enc.  Inputs             & \multicolumn{1}{l|}{225}                      & \multicolumn{1}{l|}{784}          & 3.183   \\ \hline %\cline{2-5}
Enc.  Filters            & \multicolumn{1}{l|}{149}                      & \multicolumn{1}{l|}{2384}         & 2.12  \\ \hline %\cline{2-7}
Enc.  Weights            & \multicolumn{1}{l|}{40}                       & \multicolumn{1}{l|}{640}           & 0.561   \\ \hline %\cline{2-7}
 \textbf{Total}      & \multicolumn{1}{l|}{189}                      & \multicolumn{1}{l|}{3024}         & 2.681  \\ \hline %\cline{2-7}
  CL1                & \multicolumn{1}{l|}{(1200,1225)}              & \multicolumn{1}{l|}{(92928,94864)}& 15.882 \\ \hline %\cline{2-7}
  Square             & \multicolumn{1}{l|}{25}                       & \multicolumn{1}{l|}{1936}          & 0.251    \\ \hline %\cline{2-7}
  CL2                & \multicolumn{1}{l|}{(112,100,16)}             & \multicolumn{1}{l|}{(25536,25600)}  & 0.859  \\ \hline %\cline{2-7}
  Square             & \multicolumn{1}{l|}{4}                        & \multicolumn{1}{l|}{64}            & 0.021   \\ \hline %\cline{2-7}
  FL1                & \multicolumn{1}{l|}{(110,40,80)}              & \multicolumn{1}{l|}{(630,640)}   & 0.258   \\ \hline %\cline{2-7}
 \textbf{Total}      & \multicolumn{1}{l|}{(1422,1394,96)}           & \multicolumn{1}{l|}{(119094,123104)}     &17.271 \\ \hline %\cline{2-7}
 \textbf{Amortized}  & \multicolumn{1}{l|}{(88.9,\textbf{87.1,6})}            & \multicolumn{1}{l|}{(29.1,\textbf{30.1})}  &1.079        \\ \hline
\end{tabular}
}
\end{table}

\begin{table}[htb]
\centering
\caption{LHE operations and time for {\it CNN 4-2} (Our Scheme: n=128, r=16).}
\label{tab:cnn-4-2}
\resizebox{\linewidth}{!}{
\begin{tabular}{|l|ll|l|}
\hline
                & \multicolumn{2}{c|}{LHE operations}                     & \multicolumn{1}{c|}{Time} \\ \hline
                & \multicolumn{1}{l|}{Our Scheme}         & CryptoNets      & Our Scheme                   \\ \hline
Enc. Inputs         & \multicolumn{1}{l|}{441}              & 784             & 20.036                     \\ \hline
Filters        & \multicolumn{1}{l|}{133}              & 2128            & 6.150                      \\ \hline %\cline{2-5} 
Weights        & \multicolumn{1}{l|}{320}              & 1184            & 14.471                     \\ \hline %\cline{2-5} 
\textbf{Total} & \multicolumn{1}{l|}{453}              & 3312            & 20.621                     \\ \hline
CL1            & \multicolumn{1}{l|}{(1944,2025,0)}    & (55296,57600)   & 133.093                    \\ \hline %\cline{2-5} 
Square         & \multicolumn{1}{l|}{81}               & 2304            & 4.579                      \\ \hline %\cline{2-5} 
CL2            & \multicolumn{1}{l|}{(2352,1764,784)}  & (57200,57600)   & 112.451                    \\ \hline %\cline{2-5} 
Square         & \multicolumn{1}{l|}{196}              & 400             & 7.368                      \\ \hline %\cline{2-5} 
CL3            & \multicolumn{1}{l|}{(315,324,0)}      & (8960,9216)     & 11.85                      \\ \hline %\cline{2-5} 
Square         & \multicolumn{1}{l|}{9}                & 256             & 0.222                      \\ \hline %\cline{2-5} 
CL4            & \multicolumn{1}{l|}{(48,36,16)}       & (2288,2304)     & 1.128                      \\ \hline %\cline{2-5} 
Square         & \multicolumn{1}{l|}{4}                & 16              & 0.059                      \\ \hline %\cline{2-5} 
FL1            & \multicolumn{1}{l|}{(576,256,384)}    & (960,1024)      & 5.452                      \\ \hline %\cline{2-5} 
FL2            & \multicolumn{1}{l|}{(63,64,0)}        & (150,160)       & 0.822                      \\ \hline %\cline{2-5} 
\textbf{Total} & \multicolumn{1}{l|}{(5298,4759,1184)} & (124854,130880) & 277.024                    \\ \hline %\cline{2-5} 
\textbf{Amortized}                & \multicolumn{1}{l|}{(41.4,\textbf{37.2,9.3})}                 &(15.2,\textbf{16})                 & 2.164                           \\ \hline
\end{tabular}
}
\end{table}

As in Table~\ref{tab:cnn-2-1},
when our scheme is applied to CNN 2-1 with $16$ parallel inputs,
to compute inference from the inputs takes $17.271$ seconds, which is 
$1.079$ seconds for each input. 
With the setting, 
our scheme performs $87.1$ $\otimes$ and $6$ $Rot$ operations for each of its $16$ input.
CryptoNets performs $30.1$ $\otimes$ for each of its $4096$ inputs; however,
if it has only $16$ inputs available, it performs $7705.6$ $\otimes$ operations per input,
which is around $82$ times higher.
Similar trends can be observed from Table~\ref{tab:cnn-4-2}, except that
the amortized cost increases as the scale of the model increases, which is reasonable. 
Hence, {\em our scheme has good applicability and scalability with varying size of simultaneously-available inputs under various CNN models}.    


% Table~\ref{tab:cnn-2-1} and table~\ref{tab:cnn-2-2} report the FHE operations and delay for {\it CNN 2-1} and {\it CNN 2-2} respectively.
% {\it CNN 2-1} and {\it CNN 2-2} share the same CLs and the last CL output matrix has dimension $4\times4$. In order to support the CNN depth and fully utilize the slots, we set $N=8192, n=16$ in {\it CNN 2-1} and $N=16384, n =32$ in {\it CNN 2-2}. 
% $r=1$ means the cross-filter and cross-channel packing are not applied. After applying the optimizations, the total operations and delay are greatly reduced.
% The total operations and delay in {\it CNN 2-1} is larger than in {\it CNN 2-2}. 
% When more inputs are in parallel, amortized operations are less.

% In table~\ref{tab:cnn-4-1} and table~\ref{tab:cnn-4-2}, CNNs with more layers are measured. With same polynomial modulus $N=16384$, when FHE levels is higher, the operation cost is higher. Therefore, for the same steps of encrypting inputs and models, and CLs forward propagation, {\it CNN 4-2} incurs larger delay than {\it CNN 4-1}.
% The amortized delay in {\it CNN 4-2} is 2.164 while the value is 1.87 in {\it CNN 4-1}.

% \begin{table*}[htb]
% \centering
% \caption{The FHE operations and delay for {\it CNN 2-1} on MNIST in seconds.}
% \label{tab:cnn-2-1}
% \resizebox{0.8\textwidth}{!}{
% \begin{tabular}{|l|l|lll|ll|}
% \hline
%                                       &                     & \multicolumn{3}{c|}{FHE operations}                                                                       & \multicolumn{2}{c|}{Delay}             \\ \hline
%                                       &                     & \multicolumn{1}{l|}{(16,16)}                  & \multicolumn{1}{l|}{(16,1)}               & CryptoNets    & \multicolumn{1}{l|}{(16,16)} & (16,1)  \\ \hline
% Encrypt Inputs                        &  Inputs             & \multicolumn{1}{l|}{225}                      & \multicolumn{1}{l|}{225}                  & 784           & \multicolumn{1}{l|}{3.183}   & 3.377   \\ \hline\cline{2-7}
% \multirow{3}{*}{Encrypt Models}       &  Filters            & \multicolumn{1}{l|}{149}                      & \multicolumn{1}{l|}{2384}                 & 2384          & \multicolumn{1}{l|}{2.12}    & 35.019   \\ \cline{2-7}
%                                       &  Weights            & \multicolumn{1}{l|}{40}                       & \multicolumn{1}{l|}{40}                   & 640           & \multicolumn{1}{l|}{0.561}   & 0.591   \\ \cline{2-7}
%                                       & \textbf{Total}      & \multicolumn{1}{l|}{189}                      & \multicolumn{1}{l|}{2424}                 & 3024          & \multicolumn{1}{l|}{2.681}   & 35.61         \\ \hline\cline{2-7}
% \multirow{7}{*}{Forward Propagation}  &  CL1                & \multicolumn{1}{l|}{(1200,1225)}              & \multicolumn{1}{l|}{(19200,19600)}        & (92928,94864) & \multicolumn{1}{l|}{15.882}  & 252.123 \\ \cline{2-7}
%                                       &  Square             & \multicolumn{1}{l|}{25}                       & \multicolumn{1}{l|}{400}                  & 1936          & \multicolumn{1}{l|}{0.251}   & 3.9        \\ \cline{2-7}
%                                       &  CL2                & \multicolumn{1}{l|}{(112,100,16)}             & \multicolumn{1}{l|}{(1590,1600)}          & (25536,25600) & \multicolumn{1}{l|}{0.859}   & 12.834  \\ \cline{2-7}
%                                       &  Square             & \multicolumn{1}{l|}{4}                        & \multicolumn{1}{l|}{4}                    & 64            & \multicolumn{1}{l|}{0.021}   & 0.021   \\ \cline{2-7}
%                                       &  FL1                & \multicolumn{1}{l|}{(110,40,80)}              & \multicolumn{1}{l|}{(70,40,40)}           & (630,640)     & \multicolumn{1}{l|}{0.258}   & 0.281   \\ \cline{2-7}
%                                       & \textbf{Total}      & \multicolumn{1}{l|}{(1422,1394,96)}           & \multicolumn{1}{l|}{(20860,21644,40)}     & (119094,123104)               & \multicolumn{1}{l|}{17.271}   & 269.159 \\ \cline{2-7}
%                                       & \textbf{Amortized}  & \multicolumn{1}{l|}{(88.9,87.1,6)}            & \multicolumn{1}{l|}{(1303.8,1352.8,2.5)}  &(29.1,30.1)                    & \multicolumn{1}{l|}{1.079}    & 16.822        \\ \hline

% \end{tabular}
% }
% \end{table*}

% \begin{table*}[htb]
% \centering
% \caption{The FHE operations and delay for {\it CNN 2-2} on MNIST in seconds.}
% \label{tab:cnn-2-2}
% \resizebox{0.8\textwidth}{!}{
% \begin{tabular}{|l|l|lll|ll|}
% \hline
%                                       &                     & \multicolumn{3}{c|}{FHE operations}                                                     & \multicolumn{2}{c|}{Delay}             \\ \hline
%                                       &                     & \multicolumn{1}{l|}{(32,16)}       & \multicolumn{1}{l|}{(32,1)}        & CryptoNets    & \multicolumn{1}{l|}{(32,16)} & (32,1)  \\ \hline
% Encrypt Inputs                        &  Inputs             & \multicolumn{1}{l|}{225}           & \multicolumn{1}{l|}{225}           & 784           & \multicolumn{1}{l|}{7.172}   & 7.125   \\ \hline
% \multirow{3}{*}{Encrypt Models}       &  Filters            & \multicolumn{1}{l|}{149}           & \multicolumn{1}{l|}{2384}          & 2384          & \multicolumn{1}{l|}{4.851}   & 71.089  \\ \cline{2-7}
%                                       &  Weights            & \multicolumn{1}{l|}{320}           & \multicolumn{1}{l|}{320}           & 4160          & \multicolumn{1}{l|}{10.097}  & 9.679   \\ \cline{2-7}
%                                       & \textbf{Total}      & \multicolumn{1}{l|}{469}           & \multicolumn{1}{l|}{2704}          & 6544          & \multicolumn{1}{l|}{14.948}  & 80.768         \\ \hline
% \multirow{8}{*}{Forward Propagation}  &  CL1                & \multicolumn{1}{l|}{(1200,1225)}   & \multicolumn{1}{l|}{(19200,19600)} & (92928,94864) & \multicolumn{1}{l|}{40.153}  & 642.546 \\ \cline{2-7}
%                                       &  Square             & \multicolumn{1}{l|}{25}            & \multicolumn{1}{l|}{400}           & 1936          & \multicolumn{1}{l|}{0.639}   & 10.235  \\ \cline{2-7}
%                                       &  CL2                & \multicolumn{1}{l|}{(112,100,16)}  & \multicolumn{1}{l|}{(1590,1600)}   & (25536,25600) & \multicolumn{1}{l|}{2.311}   & 34.809  \\ \cline{2-7}
%                                       &  Square             & \multicolumn{1}{l|}{4}             & \multicolumn{1}{l|}{4}             & 64            & \multicolumn{1}{l|}{0.057}   & 0.058   \\ \cline{2-7}
%                                       &  FL1                & \multicolumn{1}{l|}{(704,256,512)} & \multicolumn{1}{l|}{(448,256,256)} & (4032,4096)   & \multicolumn{1}{l|}{5.39}    & 4.441   \\ \cline{2-7}
%                                       &  FL2                & \multicolumn{1}{l|}{(63,64,0)}       & \multicolumn{1}{l|}{(63,64,0)}         & (630,640)         & \multicolumn{1}{l|}{0.607}        & 0.596   \\ \cline{2-7}
%                                       & \textbf{Total}      & \multicolumn{1}{l|}{(2079,1674,528)} & \multicolumn{1}{l|}{(21301,21924,256)} & (123126,127200)   & \multicolumn{1}{l|}{49.157}       & 692.685 \\ \cline{2-7}
%                                       & \textbf{Amortized}  & \multicolumn{1}{l|}{(65,52.3,16.5)}  & \multicolumn{1}{l|}{(665.7,685.1,8)}   & (15,15.5)         & \multicolumn{1}{l|}{1.54}          & 21.6        \\ \hline
% \end{tabular}
% }
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[htb]
% \centering
% \caption{The FHE operations and delay for {\it CNN 3-1} on MNIST in seconds.}
% \label{tab:cnn-3-1}
% \resizebox{0.8\textwidth}{!}{
% \begin{tabular}{|l|l|lll|ll|}
% \hline
%                                      &                  & \multicolumn{3}{c|}{FHE operations}                                                         & \multicolumn{2}{c|}{Delay}             \\ \hline
%                                      &                  & \multicolumn{1}{l|}{(32,16)}        & \multicolumn{1}{l|}{(32,1)}           & CryptoNets    & \multicolumn{1}{l|}{(32,16)} & (32,1)  \\ \hline
% Encrypt Inputs                       & Inputs           & \multicolumn{1}{l|}{225}            & \multicolumn{1}{l|}{225}              & 784           & \multicolumn{1}{l|}{7.671}   & 8.267   \\ \hline
% \multirow{3}{*}{Encrypt Models}      & Filters          & \multicolumn{1}{l|}{81}             & \multicolumn{1}{l|}{1296}             & 1296          & \multicolumn{1}{l|}{2.822}   & 42.555  \\ \cline{2-7} 
%                                      & Weights          & \multicolumn{1}{l|}{10}             & \multicolumn{1}{l|}{160}              & 2560          & \multicolumn{1}{l|}{0.354}   & 5.328   \\ \cline{2-7} 
%                                      & \textbf{Total}   & \multicolumn{1}{l|}{91}             & \multicolumn{1}{l|}{1456}             & 3856          & \multicolumn{1}{l|}{3.176}   & 47.883  \\ \hline
% \multirow{9}{*}{Forward Propagation} & CL1              & \multicolumn{1}{l|}{(392,441,0)}    & \multicolumn{1}{l|}{(6272,7056)}      & (21632,24336) & \multicolumn{1}{l|}{18.452}  & 288.41  \\ \cline{2-7} 
%                                      & Square           & \multicolumn{1}{l|}{49}             & \multicolumn{1}{l|}{784}              & 2704          & \multicolumn{1}{l|}{1.624}   & 25.531  \\ \cline{2-7} 
%                                      & CL2              & \multicolumn{1}{l|}{(432,324,144)}  & \multicolumn{1}{l|}{(5148,5184)}      & (20592,20736) & \multicolumn{1}{l|}{11.406}  & 139.15  \\ \cline{2-7} 
%                                      & Square           & \multicolumn{1}{l|}{36}             & \multicolumn{1}{l|}{36}               & 144           & \multicolumn{1}{l|}{0.726}   & 0.705   \\ \cline{2-7} 
%                                      & CL3              & \multicolumn{1}{l|}{(35,36,0)}      & \multicolumn{1}{l|}{(560,576,0)}      & (8960,9216)   & \multicolumn{1}{l|}{0.691}   & 9.828   \\ \cline{2-7} 
%                                      & Square           & \multicolumn{1}{l|}{1}              & \multicolumn{1}{l|}{16}               & 256           & \multicolumn{1}{l|}{0.013}   & 0.169   \\ \cline{2-7} 
%                                      & FL1              & \multicolumn{1}{l|}{(80,10,80)}     & \multicolumn{1}{l|}{(190,160,40)}     & (2550,2560)   & \multicolumn{1}{l|}{0.328}   & 1.835   \\ \cline{2-7} 
%                                      & \textbf{Total}   & \multicolumn{1}{l|}{(939,897,224)}  & \multicolumn{1}{l|}{(12170,13812,40)} & (53734,59952) & \multicolumn{1}{l|}{33.24}   & 465.628 \\ \cline{2-7}
%                                      &\textbf{Amortized}& \multicolumn{1}{l|}{(29.3,28,7)}    & \multicolumn{1}{l|}{(380.3,431.6,1.3)}&  (6.6,7.3)            & \multicolumn{1}{l|}{1.039}        & 14.551        \\ \hline
% \end{tabular}
% }
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[htb]
% \centering
% \caption{The FHE operations and delay for {\it CNN 4-1} on MNIST in seconds.}
% \label{tab:cnn-4-1}
% \resizebox{0.6\textwidth}{!}{
% \begin{tabular}{|l|l|ll|l|}
% \hline
%                                       &                & \multicolumn{2}{c|}{FHE operations}                    & \multicolumn{1}{c|}{Delay} \\ \hline
%                                       &                & \multicolumn{1}{l|}{(128,16)}        & CryptoNets      & (128,16)                   \\ \hline
% Encrypt Inputs                        & Inputs         & \multicolumn{1}{l|}{441}             & 784             & 18.867                     \\ \hline
% \multirow{3}{*}{Encrypt Models}       & Filters        & \multicolumn{1}{l|}{133}             & 2128            & 5.804                      \\ \cline{2-5} 
%                                       & Weights        & \multicolumn{1}{l|}{40}              & 160             & 1.701                      \\ \cline{2-5} 
%                                       & \textbf{Total} & \multicolumn{1}{l|}{173}             & 2288            & 7.505                      \\ \hline
% \multirow{11}{*}{Forward Propagation} & CL1            & \multicolumn{1}{l|}{(1944,2025,0)}   & (55296,57600)   & 119.634                    \\ \cline{2-5} 
%                                       & Square         & \multicolumn{1}{l|}{81}              & 2304            & 4.078                      \\ \cline{2-5} 
%                                       & CL2            & \multicolumn{1}{l|}{(2352,1764,784)} & (57200,57600)   & 97.623                     \\ \cline{2-5} 
%                                       & Square         & \multicolumn{1}{l|}{196}             & 400             & 6.588                      \\ \cline{2-5} 
%                                       & CL3            & \multicolumn{1}{l|}{(315,324,0)}     & (8960,9216)     & 9.653                      \\ \cline{2-5} 
%                                       & Square         & \multicolumn{1}{l|}{9}               & 256             & 0.188                      \\ \cline{2-5} 
%                                       & CL4            & \multicolumn{1}{l|}{(48,36,16)}      & (2288,2304)     & 0.885                      \\ \cline{2-5} 
%                                       & Square         & \multicolumn{1}{l|}{4}               & 16              & 0.045                      \\ \cline{2-5} 
%                                       & FL1            & \multicolumn{1}{l|}{(90,40,60)}      & (150,160)       & 0.647                      \\ \cline{2-5} 
%                                       & \textbf{Total} & \multicolumn{1}{l|}{(4749,4479,860)} & (123894,129856) & 239.341                    \\ \cline{2-5} 
%                                       &\textbf{Amortized}      & \multicolumn{1}{l|}{(37.1,35,6.7)}   &(15.1,15.9)                 &   1.87                         \\ \hline
% \end{tabular}
% }
% \end{table*}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \begin{table*}[htb]
% \centering
% \caption{The FHE operations and delay for {\it CNN 4-2} on MNIST in seconds.}
% \label{tab:cnn-4-2}
% \resizebox{0.6\textwidth}{!}{
% \begin{tabular}{|l|l|ll|l|}
% \hline
%                                       &                & \multicolumn{2}{c|}{FHE operations}                     & \multicolumn{1}{c|}{Delay} \\ \hline
%                                       &                & \multicolumn{1}{l|}{(128,16)}         & CryptoNets      & (128,16)                   \\ \hline
% Encrypt Inputs                        & Inputs         & \multicolumn{1}{l|}{441}              & 784             & 20.036                     \\ \hline
% \multirow{3}{*}{Encrypt Models}       & Filters        & \multicolumn{1}{l|}{133}              & 2128            & 6.150                      \\ \cline{2-5} 
%                                       & Weights        & \multicolumn{1}{l|}{320}              & 1184            & 14.471                     \\ \cline{2-5} 
%                                       & \textbf{Total} & \multicolumn{1}{l|}{453}              & 3312            & 20.621                     \\ \hline
% \multirow{12}{*}{Forward Propagation} & CL1            & \multicolumn{1}{l|}{(1944,2025,0)}    & (55296,57600)   & 133.093                    \\ \cline{2-5} 
%                                       & Square         & \multicolumn{1}{l|}{81}               & 2304            & 4.579                      \\ \cline{2-5} 
%                                       & CL2            & \multicolumn{1}{l|}{(2352,1764,784)}  & (57200,57600)   & 112.451                    \\ \cline{2-5} 
%                                       & Square         & \multicolumn{1}{l|}{196}              & 400             & 7.368                      \\ \cline{2-5} 
%                                       & CL3            & \multicolumn{1}{l|}{(315,324,0)}      & (8960,9216)     & 11.85                      \\ \cline{2-5} 
%                                       & Square         & \multicolumn{1}{l|}{9}                & 256             & 0.222                      \\ \cline{2-5} 
%                                       & CL4            & \multicolumn{1}{l|}{(48,36,16)}       & (2288,2304)     & 1.128                      \\ \cline{2-5} 
%                                       & Square         & \multicolumn{1}{l|}{4}                & 16              & 0.059                      \\ \cline{2-5} 
%                                       & FL1            & \multicolumn{1}{l|}{(576,256,384)}    & (960,1024)      & 5.452                      \\ \cline{2-5} 
%                                       & FL2            & \multicolumn{1}{l|}{(63,64,0)}        & (150,160)       & 0.822                      \\ \cline{2-5} 
%                                       & \textbf{Total} & \multicolumn{1}{l|}{(5298,4759,1184)} & (124854,130880) & 277.024                    \\ \cline{2-5} 
%                                       &\textbf{Amortized}                & \multicolumn{1}{l|}{(41.4,37.2,9.3)}                 &(15.2,16)                 & 2.164                           \\ \hline
% \end{tabular}
% }
% \end{table*}




% \begin{table*}[htb]
% \centering
% \caption{LHE operations for {\it CNN 2-2} (Our Scheme: n=32, r=16).}
% \label{tab:cnn-2-2}
% \resizebox{0.8\textwidth}{!}{

% \begin{tabular}{|l|ll|l|}
% \hline
%                      & \multicolumn{2}{c|}{LHE Operations}                           & \multicolumn{1}{c|}{Time}             \\ \hline
%                      & \multicolumn{1}{l|}{Our Scheme}                  & \multicolumn{1}{l|}{CryptoNets}   & Our Scheme  \\ \hline
% Enc.  Inputs             & \multicolumn{1}{l|}{225}                      & \multicolumn{1}{l|}{784}          & 7.172   \\ \hline %\cline{2-5}
% Enc.  Filters            & \multicolumn{1}{l|}{149}                      & \multicolumn{1}{l|}{2384}         & 4.851  \\ \hline %\cline{2-7}
% Enc.  Weights            & \multicolumn{1}{l|}{320}                       & \multicolumn{1}{l|}{4160}           & 10.097   \\ \hline %\cline{2-7}
%  \textbf{Total}      & \multicolumn{1}{l|}{469}                      & \multicolumn{1}{l|}{6544}         & 14.948  \\ \hline %\cline{2-7}
%   CL1                & \multicolumn{1}{l|}{(1200,1225)}              & \multicolumn{1}{l|}{(92928,94864)}& 40.153 \\ \hline %\cline{2-7}
%   Square             & \multicolumn{1}{l|}{25}                       & \multicolumn{1}{l|}{1936}          & 0.639    \\ \hline %\cline{2-7}
%   CL2                & \multicolumn{1}{l|}{(112,100,16)}             & \multicolumn{1}{l|}{(25536,25600)}  & 2.311  \\ \hline %\cline{2-7}
%   Square             & \multicolumn{1}{l|}{4}                        & \multicolumn{1}{l|}{64}            & 0.057   \\ \hline %\cline{2-7}
%   FL1                & \multicolumn{1}{l|}{(704,256,512)}              & \multicolumn{1}{l|}{(4032,4096)}   & 5.39   \\ \hline %\cline{2-7}
%   FL2                & \multicolumn{1}{l|}{(63,64,0)}              & \multicolumn{1}{l|}{(630,640)}   & 0.607   \\ \hline %\cline{2-7}
%  \textbf{Total}      & \multicolumn{1}{l|}{(2079,1674,528)}           & \multicolumn{1}{l|}{(123126,127200)}     &49.157 \\ \hline %\cline{2-7}
%  \textbf{Amortized}  & \multicolumn{1}{l|}{(65,\textbf{52.3,16.5})}            & \multicolumn{1}{l|}{(15,\textbf{15.5})}  &1.54       \\ \hline
% \end{tabular}

% }
% \end{table*}

==> integrity.tex <==
\section{Scheme for Testing Computation Integrity}
\label{sec:integrity}



==> optimize.tex <==
\section{Optimizations on Packing}
\label{sec:optimize}

With the above scheme,
each initial input ciphertext encodes/encrypts $n\cdot\tilde{\beta}_0^2$ input values.
If $n\cdot\tilde{\beta}_0^2$ is much less than ${\cal S}$ (i.e., the number of available slots in a ciphertext),
the slots will not be effectively utilized and the computation/communication efficiency will be negatively affected.
To address this limitation, we propose cross-channel and cross-filter packing in this section.
%
% When the number of available data sets $n$ is small or the slots number $s$ is much larger than $n\cdot\tilde{\beta}_0^2$, in order to fully utilize the slots in a ciphertext, we propose two ways to optimize the packing methods of the convolutional layer from the basic scheme. 
%
Specifically, 
letting $r$ be the largest power of two which is no greater than $\frac{\cal S}{n\cdot\tilde{\beta}_0^2}$, 
the inputs from $r$ channels can be encoded together such that more input values can be processed in parallel, 
or each ciphertext can encode/encrypt $r$ replicas of the original $n\cdot\tilde{\beta}_0^2$ values such that
the same input can be processed with multiple filters in parallel. 
Such changes, however, also demand according changes to the procedure of propagation through each convolutional layer.
In this section, we elaborate on these optimizations. 

%In this section, we elaborate the methods to parallel channels and filters in convolutional layer $l$.

\subsection{Cross-Channel Packing}

With cross-channel packing,
input values from $r$ different channels can be encoded/encrypted 
% Multiple ciphertexts of different channels can be combined 
into one ciphertext; accordingly,
the elements of the filters associated with these channels should be encoded together accordingly.  
% the corresponding ciphertexts for filter matrix elements should be combined accordingly.
Such a design reduces the number of input ciphertexts at convolutional layer $l$ to 
$\tilde{\gamma}_l^2\lceil\frac{\alpha_l}{r} \rceil$ and reduces  
the number of ciphertexts that encode/encrypt filters to $\epsilon_l\lceil\frac{\alpha_l}{r} \rceil\beta_l^2$.

More specifically,  
all the $\alpha_l$ channels at layer $l$ are grouped into $\lceil\frac{\alpha_l}{r}\rceil$ groups,
where each channel group $i'$ includes channels $\{i'\cdot r,\cdots,\min\{(i'+1)\cdot r,\alpha_0\}-1\}$.
%
All the plaintext input values to this layer are now encoded/encrypted into ciphertexts 
$\vec{C}^{(l)}_{i',u,v}$ for every $i'\in\{0,\cdots,\lceil\frac{\alpha_l}{r}\rceil-1\}$
and every $(u,v)\in\{0,\cdots,\tilde{\gamma}_l-1\}^2$.
Here, each $\vec{C}^{(l)}_{i',u,v}$ encodes/encrypts the concatenation of $r$ vectors formatted as as 
Eq.~(\ref{eq:initial-input-format-1}) and (\ref{eq:initial-input-format-2})
for every $i\in\{i'\cdot r,\cdots,\min\{(i'+1)\cdot r,\alpha_l\}-1\}$.
%
Accordingly, for every $i'$, every $k\in\{0,\epsilon_l-1\}$ and every $(x,y)\in\{0,\cdots,\beta_l-1\}^2$,
a ciphertext $\hat{F}^{(l,k)}_{i',x,y}$ is constructed to encode/encrypt 
the elements with index $(x,y)$, which is replicated for $n$ copies, of the $k$-th filers in every channels of channel group $i'$.

Based on the above encryption strategy,
the procedure of propagation through this layer is formalized in Algorithm~\ref{alg:fwd-conv-layer-cross-channels}.
%
As we can see, most part of this algorithm is similar to Algorithm~\ref{alg:fwd-conv-layer}, but it
reduces the iteration number from $\alpha_l$ to $\lceil\frac{\alpha_l}{r}\rceil$ in the innermost layer of loop (lines 6-9).
The algorithm further employs rotation to sum up subsets of the elements encoded/encrypted in each ciphertext,
which is similar to Algorithm~\ref{alg:fwd-full-layer-I}.
%
Each ciphertext output by this algorithm contains $r$ replicas of data set encoded/encrypted in the cross-filter pattern.
If the output is used as the input of next convolutional layer,
they can be processed as described next. 





% the element with the same index $(u,v)$ in every filter matrix of a set of $r$ channels 
% are each duplicated for $n\cdot\tilde{\beta}_l^2$ times and then concatenated to form a vector,
% which is then encoded/encrypted to a ciphertext.



% now encodes/encrypts the concatenation of $r$ vectors each is formatted as 

% the new ciphertext $\vec{C}_{i,u,v}$ encrypts the concatenation of vectors: $(\vec{I}_{i\cdot r,u,v},\vec{I}_{i\cdot r+1,u,v},\cdots,\vec{I}_{\min\{(i+1)\cdot r, \alpha_l\}-1,u,v})$ for each 
% $i\in\{0,\cdots,\lceil\frac{\alpha_l}{r}\rceil-1\}$ and each $u,v\in\{0,\cdots,\tilde{\gamma}_l-1\}$;
% correspondingly, for each pair $(u,v)$ where $u,v\in\{0,\cdots,\beta_l-1\}$,
% the element with the same index $(u,v)$ in each of filter matrices of $r$ parallel channels 
% are each duplicated for $n\cdot\tilde{\beta}_0^2$ times and then concatenated to form a vector,
% which is then encrypted to a ciphertext.
% To be specific, assume $\vec{F}^{(l,k)}_{j,u,v}=(F_{k,j,u,v},\cdots, F_{k,j,u,v})$ that is to have $k$-th filter with element index $(u,v)$ in channel $j\in\{0,\cdots,\alpha_l-1\}$ repeated $n\cdot\tilde{\beta}^2_0$ times. 
% Then each ciphertext $\hat{F}^{(l,k)}_{i,u,v}$ encrypts the concatenation of vectors:
% $(\vec{F}^{(l,k)}_{ir,u,v},\vec{F}^{(l,k)}_{ir+1,u,v},\cdots,\vec{F}^{(l,k)}_{\min\{(i+1)r,\alpha_l\}-1,u,v})$
% where $k\in\{0,\cdots,\epsilon_l-1\}$ and $i\in\{0,\cdots,\lceil\frac{\alpha_l}{r}\rceil-1\}$. 


% Algorithm~\ref{alg:fwd-conv-layer-cross-channels} formally presents how the forward propagation is conducted
% through a convolutional layer $l$ with the optimized cross channels packing.
% The convolutional layer output ciphertext $\tilde{C}^{(l+1)}_{k,u,v}$ has the format of encoding $n\cdot\tilde{\beta}_0^2$ different values and each repeats $r$ times which leads to the cross filters packing as the duplicated values can be utilized for parallel computation by the same element from different filters.

\begin{algorithm}[htb]
\SetAlgoLined
\caption{Propagation Through Convolutional Layer $l$ with Cross-Channel Packing}
\label{alg:fwd-conv-layer-cross-channels}

\For{$k\in\{0,\cdots,\epsilon_l-1\}$}{ %\Comment{$\epsilon_l=\alpha_{l+1}$ each output channel}
    \For{$(u,v)\in\{0,\cdots,\tilde{\gamma}_{l+1}-1\}^2$}{
        $\hat{C}^{(l+1)}_{k,u,v}\leftarrow 0$; \Comment{each element of output matrix}\;
        $(u',~v')\leftarrow (\delta_l\cdot u,~\delta_l\cdot v)$\;
        \For{$(x,y)\in\{0,\cdots,\gamma_l-1\}^2$}{
            \For{$i'\in\{0,\cdots,\lceil\frac{\alpha_l}{r}\rceil-1\}$}{ 
                \Comment{iterating each channel group}\;
                $\hat{C}^{(l+1)}_{k,u,v} \oplus= \hat{C}^{(l)}_{i',u'+x,v'+y}\otimes \hat{F}^{(l,k)}_{i',x,y}$;
            }
        }
        \For{$j\in\{1,\cdots,\log(r)\}$}{ %\Comment{sum up all channels}
                $\tilde{C}^{(l+1)}_{k,u,v} += Rot(\tilde{C}^{(l+1)}_{k,u,v},~j\cdot n\cdot\tilde{\beta}_0^2)$;
        }
        $\hat{C}^{(l+1)}_{k,u,v}\leftarrow \hat{C}^{(l+1)}_{k,u,v}\otimes\hat{C}^{(l+1)}_{k,u,v}$; 
                \Comment{activation}
    }
}

\end{algorithm}



 
% \begin{algorithm}[htb]
% \caption{Propagation Through Convolutional Layer $l$ with Cross Channels Packing}
% \label{alg:fwd-conv-layer-cross-channels}

% \begin{algorithmic}[1]

% \For{$k\in\{0,\cdots,\epsilon_l-1\}$} \Comment{$\epsilon_l=\alpha_{l+1}$ each output channel}
%     \For{$u\in\{0,\cdots,\tilde{\gamma}_{l+1}-1\}$}
%         \For{$v\in\{0,\cdots,\tilde{\gamma}_{l+1}-1\}$} 
%             \State $\tilde{C}^{(l+1)}_{k,u,v}\leftarrow 0$ \Comment{each element of output matrix}
%             \State $u'\leftarrow \delta_l\cdot u$
%             \State $v'\leftarrow \delta_l\cdot v$
%             \For{$x\in\{0,\cdots,\gamma_l-1\}$}
%                 \For{$y\in\{0,\cdots,\gamma_l-1\}$}
%                     \For{$i\in\{0,\cdots,\lceil\frac{\alpha_l}{r}\rceil-1\}$} \Comment{each cross channels packing}
%                     \State $\tilde{C}^{(l+1)}_{k,u,v} += \tilde{C}^{(l)}_{i,u'+x,v'+y}\bigodot \hat{F}^{(l,k)}_{i,x,y}$
%                     \EndFor
%                 \EndFor
%             \EndFor
%             \For{$j\in\{1,\cdots,\log(r)\}$} \Comment{sum up all channels}
%                 \State $\tilde{C}^{(l+1)}_{k,u,v} += Rotate(\tilde{C}^{(l+1)}_{k,u,v},j\cdot n\cdot\tilde{\beta}_0^2)$
%             \EndFor
%         \EndFor
%     \EndFor
% \EndFor

% \end{algorithmic}
% \end{algorithm}

\subsection{Cross-Filter Packing}

With cross-filter packing,
distinct input values are packed as pi-sets and then all these distinct values 
as whole is replicated for $r$ times.
Specifically for a layer $l$ with cross-filter packing input,
the input includes $\alpha_l\cdot\tilde{\gamma}_l^2$ ciphertexts. 
Each ciphertext $\hat{C}^{(l)}_{i,u,v}$ for channel $i\in\{0,\cdots,\alpha_l-1\}$
and $(u,v)\in\{0,\cdots,\tilde{\gamma}_l-1\}^2$ encodes/encrypts 
$r$ replicas of the $\tilde{\beta}_l$ pi-sets 
that are formatted similarly to Eq.~(\ref{eq:initial-input-format-1}) and (\ref{eq:initial-input-format-2}).

The existence of replication in the ciphertexts provides an opportunity for 
each ciphertext to be multiplied with a ciphertext encoding/encrypting elements from multiple filters at a time;
this way, increased level of parallel processing can be attained. 
%
Specifically, for each channel $i$, all the $\epsilon_l$ filter matrices are grouped into $\lceil\frac{\epsilon_l}{r}\rceil$ groups
such that each group $k'\in\{0,\cdots,\lceil\frac{\epsilon_l}{r}\rceil-1\}$ contains 
filters $\vec{F}^{(l,k)}$ for every $k\in\{k'\cdots r, \cdots, \min\{(k+1)\cdot r, \epsilon_l\}-1\}$. 
Then, for every such filter group $k'$ and every pair $(x,y)\in\{0,\cdots,\beta_l-1\}^2$,
a ciphertext $\hat{F}^{(l,k')}_{i,x,y}$ is constructed to encode/encrypt every element with index $(x,y)$, 
which is replicated for $n$ copies, of every filters in group $k'$ of channel $i$.

Based on the above encoding/encryption strategy, 
the propagation through this layer is formalized in Algorithm~\ref{alg:fwd-conv-layer-cross-filters}. 
%
This algorithm is similar to Algorithm~\ref{alg:fwd-conv-layer}, 
except for that it iterates through filter groups (each containing up to $r$ filters) instead of individual filters;
this way, we can gain a speed-up up to a factor of $r$. 
%
Interestingly,
the output ciphertexts, when used as input for next layer,
become cross-channel packed,
which can thus be processed as described in the previous subsection. 


% In this case, each convolutional input ciphertext is duplicated inside for multiple times; 
% accordingly, the elements from multiple filter matrices that need to be multiplied with the ciphertexts should be combined. This optimization reduces the number of filter ciphertext to $\lceil\frac{\epsilon_l}{r} \rceil\alpha_l\beta_l^2$ and the number of convolutional input ciphertexts remains to be $\tilde{r}_l^2\alpha_l$. 
% Specifically, each input ciphertext $\vec{C}_{i,u,v}$ encrypts the concatenation of vectors: $(\vec{I}_{i,u,v},\vec{I}_{i,u,v},\cdots,\vec{I}_{i,u,v})$ where $\vec{I}_{i,u,v}$ repeats $r$ times for each 
% $i\in\{0,\cdots,\alpha_l-1\}$ and each $u,v\in\{0,\cdots,\tilde{\gamma}_l-1\}$.
% For the filters packing, each element with the same index $(u,v)$ and same channel but from different filter matrices are packed together and encrypted into one ciphertext.
% That is, each ciphertext $\hat{F}^{(l,k)}_{i,u,v}$ encrypts the concatenation of vectors:
% $(\vec{F}^{(l,kr)}_{i,u,v},\vec{F}^{(l,kr+1)}_{i,u,v},\cdots,\vec{F}^{(l,\min\{(k+1)r, \epsilon_l\}-1)}_{i,u,v})$
% where $k\in\{0,\cdots,\lceil\frac{\epsilon_l}{r}\rceil-1\}$ and $i\in\{0,\cdots,\alpha_l-1\}$. 

% The convolutional layer $l$ forward propagation with the packing filters optimization is described in algorithm~\ref{alg:fwd-conv-layer-cross-filters}. 
% Compared with the basic scheme of algorithm~\ref{alg:fwd-conv-layer}, the cross filters packing parallel multiple filters into one ciphertext which reduce the number of filter ciphertexts and the computation cost in the convolutional layer.
% The convolutional results pack $r$ channels together into one ciphertext which has the same format of the cross channels packing. By applying the cross filters and crosss channels packing alternately in the convolutional layer, more slots can be further fullfilled and less ciphertexts and computation operations are required in the forward propagation.      


\begin{algorithm}[htb]
\SetAlgoLined
\caption{Propagation Through Convolutional Layer $l$ with Cross-Filter Packing}
\label{alg:fwd-conv-layer-cross-filters}

% \For{$k\in\{0,\cdots,\lceil\frac{\epsilon_l}{r}\rceil-1\}$}{ %\Comment{each cross filters packing}
%   Same as Lines $ 2-10$ in algorithm~\ref{alg:fwd-conv-layer};
% }

\For{$k'\in\{0,\cdots,\lceil\frac{\epsilon_l}{r}\rceil-1\}$}{
        \Comment{iterating each filter group}\;
        \For{$(u,~v)\in\{0,\cdots,\tilde{\gamma}_{l+1}-1\}^2$}{
                $\hat{C}^{(l+1)}_{k',u,v}\leftarrow 0$; 
                \Comment{initialize each output}\;
                $(u',~v')\leftarrow (\delta_l\cdot u,~\delta_l\cdot v)$\;
                \For{$(x,~y)\in\{0,\cdots,\gamma_l-1\}^2$}{
                        \For{$i\in\{0,\cdots,\alpha_l-1\}$}{ 
                            $\hat{C}^{(l+1)}_{k',u,v}\oplus = \hat{C}^{(l)}_{i,u'+x,v'+y}\otimes\hat{F}^{(l,k')}_{i,x,y}$;
                        }
                }
                $\hat{C}^{(l+1)}_{k',u,v}\leftarrow \hat{C}^{(l+1)}_{k',u,v}\otimes\hat{C}^{(l+1)}_{k',u,v}$; 
                \Comment{activation}
        }
}


\end{algorithm}



% \begin{algorithm}[htb]
% \caption{Propagation Through Convolutional Layer $l$ with Cross Filters Packing}
% \label{alg:fwd-conv-layer-cross-filters}

% \begin{algorithmic}[1]

% \For{$k\in\{0,\cdots,\lceil\frac{\epsilon_l}{r}\rceil-1\}$} \Comment{each cross filters packing}
%   \State Same as Lines $ 2-10$ in algorithm~\ref{alg:fwd-conv-layer}
% \EndFor

% \end{algorithmic}
% \end{algorithm}

==> scheme.tex <==

\section{LHE-based Inference Scheme}
\label{sec:scheme}

To support confidentiality-preserving inference with a CNN model 
of $c$ convolutional layers and $f$ fully connected layers,
the TEE first determines the highest encryption level ${\cal L}$ 
based on the topology of the model.
Specifically, if each layer consumes two encryption levels (as for the CNN model specified in Sec. \ref{subsec:cnn-model}),
it can set ${\cal L}=2(c+f)$. Next, the TEE 
initializes an LHE system by calling $KeyGen(2^\lambda,{\cal L})$ to obtain the keys; note that,
we set security parameter $\lambda$ to $128$ in our implementation. 
The public and evaluation keys are then distributed to the Server's REE and the clients,
while the private key is kept only by the TEE.

% as the highest encryption level and
% each ciphertext has ${\cal S}$ slots (i.e., it can encrypt up to ${\cal S}$ packed values).
% Here, ${\cal L}$ and ${\cal S}$ are derived from a certain security parameter $\lambda$,
% which is set to $128$ in our implementation. 

\subsection{Encoding and Encrypting Input Data and Filters}\label{sec:encoding}

In Steps \textcircled{3} and \textcircled{7} of the proposed framework,
the model provider should encode and encrypt its model parameters, 
and the data provider should encode and encrypt its input data,
before they upload them to the server.
%
% and the initial model parameters 
% (including the weights for filters and for fully-connected matrices), and
% then outsources them for the server to train the model. 
%
% The encoding and encryption should meet the following expectations:
% % \begin{itemize}
% %     \item 
%     after encoding and encryption, the data can be processed 
%     efficiently through the whole inference procedure, 
%     without decryption or re-encryption in the middle;
%     % \item
%     the slots available in a ciphertext should be used as much as possible 
%     for a high degree of parallel processing.
    %
    % \item
    % The ways that the weights are encoded and encrypted should facilitate efficient updating of them during the backward propagation.
    %
% \end{itemize}

% \subsubsection{Encoding and Encryption of Training Data}

\subsubsection{The Rationale}

To understand our proposed design, 
let us first briefly review the packing method in E2DM~\cite{jiang2018secure}.
We start with the simplest scenario where 
there is only one channel and one input matrix $I$ with $\beta_0^2$ values.
Following the notations introduced in Section~\ref{subsec:cnn-model},
let the only convolutional layer have kernel side $\gamma_0$ and stride $\delta_0$.
The method packs the $\beta_0^2$ values into $\gamma_0^2$ ciphertexts.
Denoting the ciphertexts as $\hat{C}_{i,j}$ for every $(i,j)\in\{0,\cdots,\gamma_0-1\}^2$,
each $\hat{C}_{i,j}$ encrypts the vector that packs all the values $I_{u,v}$ 
where $u-i$ and $v-j$ are multiples of stride $\delta_0$.
Accordingly, each element $F_{i,j}$ of each filter matrix $F$ is 
replicated to fill a vector and then encoded/encrypted to ciphertext $\hat{F}_{i,j}$; 
propagating through this layer results in a ciphertext $\sum_{0\leq i,j\leq\gamma_0-1}\hat{C}_{i,j}\otimes\hat{F}_{i,j}$. 
Note that, when there are multiple input matrices for a channel,
the above method can be straightly extended to have each ciphertext $\hat{C}_{i,j}$ 
pack and encrypt all the values $I_{u,v}$ from every input matrices $I$ 
where $u-i$ and $v-j$ are multiples of $\delta_0$.

% According to the notations introduced in Section~\ref{subsec:cnn-model}, 
% each input matrix is of $\beta_0^2$ elements.
% After one layer of filtering, it is reduced to an output matrix of $\beta_1^2$ elements,
% where $\beta_1 = 1 + \lfloor\frac{\beta_0-\gamma_0}{\delta_0}\rfloor$.
% To generalize, each convolutional layer $l$ reduces 
% an input matrix of $\beta_l^2$ elements to an output matrix of $\beta_{i+1}^2$ elements,
% where $\beta_{l+1}=1+\lfloor\frac{\beta_l-\gamma_l}{\delta_l}\rfloor$.

% \paragraph{Intuition}
To facilitate propagation through all the $c$ convolutional layers 
with packing/encryption only needed at the very beginning,
intuitively, we aim to encode/encrypt each input matrix 
as if there were only one {\em combined layer} 
that virtually includes all the $c$ layers in order.
We denote the parameters of the combined layer as:
\begin{itemize}
    \item 
    $\tilde{\delta}_0$ for {\em combined stride}, and
    \item 
    $\tilde{\gamma}_0$ for {\em combined kernel side} (i.e., $\tilde{\gamma}_0^2$ is the number of encrypted inputs for each channel).    
\end{itemize}
For convenience, we extend this notation and 
treat the combination of sequential layers from $l$ (where $0\leq l<c$) to $c-1$ as {\em combined layer from $l$};
thus, $\tilde{\delta}_l$ denotes {\em combined stride} and
$\tilde{\gamma}_l$ denotes {\em combined kernel side} for such a combined layer.

In our proposed design,
we aim to pack and encrypt data in a way that 
should meet the following requirements at each convolutional layer $l$:
%
First, $\tilde{\gamma}_l\geq\gamma_l$;
this is necessary as the input values should be 
multiplied with $\gamma_l^2$ elements of each filter respectively. 
%
Second, due to the rule of forward propagation through a convolutional layer, 
following relation should hold for 
the side $\tilde{\gamma}_l$ of each encrypted input matrix 
and the side of each output matrix (which is also the side $\tilde{\gamma}_{l+1}$
of each encrypted input matrix for layer $l+1$ when $l<c-1$):
\begin{equation}\scriptsize
    \tilde{\gamma}_{l+1} = 1 + \lfloor\frac{\tilde{\gamma}_l-\gamma_l}{\delta_l}\rfloor.
\end{equation}
%
Third, also due to the rule of the forward propagation,
following relation should hold between $\tilde{\delta}_l$
and $\tilde{\delta}_{l+1}$:
\begin{equation}\scriptsize
    \tilde{\delta}_l = \delta_l\cdot\tilde{\delta}_{l+1}.
\end{equation}
Particularly for the last convolutional layer, 
% \begin{equation}
    $\tilde{\delta}_{c-1} = \delta_{c-1}$.
% \end{equation}
%
Setting $\tilde{\gamma}_{c-1}=\gamma_{c-1}$ and guided by the above requirements,
we can derive the following general settings of the parameters for each layer $l$:
\begin{equation}\scriptsize
    \tilde{\gamma}_l = 1 + \sum_{i=l}^{c-1}(\gamma_i-1)\prod_{j=0}^{i-1}\delta_j,
\end{equation}
and 
% \begin{equation}\scriptsize
    $\tilde{\delta}_l = \prod_{i=l}^{c-1}\delta_i$.
% \end{equation}
Based on the above parameter settings, 
we elaborate our proposed method for encoding and encryption in the following. 

% the stride is the product of all the layers' strides; that is,  
% \begin{equation}
%     \tilde{\delta}_0 = \prod_{i=0}^{c-1}\delta_i,
% \end{equation}
% which we call {\em combined stride}.
% Hence, the corresponding {\em combined kernel} has side $\tilde{\gamma}_0$ 
% where 
% \begin{equation}
%     \tilde{\gamma}_0 = 1 + \sum_{i=0}^{c-1}(\gamma_i-1)\prod_{j=0}^{i-1}\delta_j,
% \end{equation}
% and accordingly, each {\em encoded input matrix} (i.e., {\em combined matrix}) 
% has side $\tilde{\beta}_0$ 
% where
% \begin{equation}
%     \tilde{\beta}_0 = 1 + \lfloor\frac{\beta_0 - \tilde{\gamma}_0}{\tilde{\delta}_0}\rfloor.
% \end{equation}

\subsubsection{Encoding and Encrypting Input Data}

For each channel $i$, 
all of its $n$ input matrices are encoded as follows.
%
Let these matrices be denoted as $I_i^{(j)}$ for every $j\in\{0,\cdots,n-1\}$, and 
each value of $I_i^{(j)}$ be denoted as $I^{(j)}_{i,x,y}$ for $x,y\in\{0,\cdots,\beta_0-1\}$.
All the values are encoded/encrypted into $\tilde{\gamma}_0^2$ ciphertexts,
each indexed by $(i,u,v)$ for $(u,v)\in\{0,\cdots,\tilde{\gamma}_0-1\}^2$.
Each ciphertext $\hat{C}^{(0)}_{i,u,v}$ encodes/encrypts the following vector:

\begin{equation}\scriptsize
\resizebox{\linewidth}{!}{
$\displaystyle
    \begin{pmatrix}\label{eq:initial-input-format-1}
        \vec{I}_{i,u,v} & \vec{I}_{i,u,v+\tilde{\delta}_0} & \cdots & \vec{I}_{i,u,v+(\tilde{\beta}_0-1)\tilde{\delta}_0} \\
        \vec{I}_{i,u+\tilde{\delta}_0,v} & 
        \vec{I}_{i,u+\tilde{\delta}_0,v+\tilde{\delta}_0} 
        & \cdots 
        & \vec{I}_{i,u+\tilde{\delta}_0,v+(\tilde{\beta}_0-1)\tilde{\delta}_0} \\
        \vdots & \vdots & \ddots & \vdots \\
        \vec{I}_{i,u+(\tilde{\beta}_0-1)\tilde{\delta}_0,v} & 
        \vec{I}_{i,u+(\tilde{\beta}_0-1)\tilde{\delta}_0,v+\tilde{\delta}_0} & 
        \cdots & 
        \vec{I}_{i,u+(\tilde{\beta}_0-1)\tilde{\delta}_0,v+(\tilde{\beta}_0-1)\tilde{\delta}_0}
    \end{pmatrix},
$
}
\end{equation}
where for each $(x,y)\in\{0,\cdots,\tilde{\gamma}_0-1\}^2$,
\begin{equation}\label{eq:initial-input-format-2}\scriptsize
    \vec{I}_{i,x,y} = ({I}_{i,x,y}^{(0)},~\cdots,~{I}_{i,x,y}^{(n-1)}).
\end{equation}

% \begin{equation}\label{eq:ciphtext-iuv}
%     \vec{I}_{i,u,v} = (\vec{I}_{i,u,v}^{(0)},~\cdots,~\vec{I}_{i,u,v}^{(n-1)}),
% \end{equation}
% where each $\vec{I}_{i,u,v}^{(j)}$ for $j\in\{0,\cdots,n-1\}$ has $\tilde{\beta}_0^2$ values as follows:
% \begin{equation}
% \resizebox{\linewidth}{!}{
% $\displaystyle
%     \begin{pmatrix}\label{eq:ciphertext-ij-detail}
%         I^{(j)}_{i,u,v} & I^{(j)}_{i,u,v+\tilde{\delta}_0} & \cdots & I^{(j)}_{i,u,v+(\tilde{\beta}_0-1)\tilde{\delta}_0} \\
%         I^{(j)}_{i,u+\tilde{\delta}_0,v} & 
%         I^{(j)}_{i,u+\tilde{\delta}_0,v+\tilde{\delta}_0} 
%         & \cdots 
%         & I^{(j)}_{i,u+\tilde{\delta}_0,v+(\tilde{\beta}_0-1)\tilde{\delta}_0} \\
%         \vdots & \vdots & \ddots & \vdots \\
%         I^{(j)}_{i,u+(\tilde{\beta}_0-1)\tilde{\delta}_0,v} & 
%         I^{(j)}_{i,u+(\tilde{\beta}_0-1)\tilde{\delta}_0,v+\tilde{\delta}_0} & 
%         \cdots & 
%         I^{(j)}_{i,u+(\tilde{\beta}_0-1)\tilde{\delta}_0,v+(\tilde{\beta}_0-1)\tilde{\delta}_0}
%     \end{pmatrix}.
% $}
% \end{equation}

% Note: To facilitate efficient summation in our designed backward propagation, 
% we assume $\tilde{\beta}_0^2$ to be a factor of $s$; if this is not the case,
% dummies can be appended at the end of the above vector to make the case.

% elements:
% \begin{equation}
%     \begin{pmatrix}
%         \vec{I}_{0,0} & \vec{I}_{0,\delta} & \cdots & \vec{I}_{0,(\beta-1)\delta} \\
%         \vec{I}_{\delta,0} & \vec{I}_{\delta,\delta} & \cdots & \vec{I}_{\delta,(\beta-1)\delta} \\
%         \vdots & \vdots & \ddots & \vdots \\
%         \vec{I}_{(\beta-1)\delta,0} & \vec{I}_{(\beta-1)\delta,\delta} & \cdots & \vec{I}_{(\beta-1)\delta,(\beta-1)\delta}
%     \end{pmatrix}
% \end{equation}
% where each sub-vector $\vec{I}_{x,y}$ for $x,y\in\{0,\delta,\cdots,(\beta-1)\delta\}$ is as follows:
% \begin{equation}
%     \vec{I}_{x,y} = (I^{(0)}_{x,y}, I^{(1)}_{x,y}, \cdots, I^{(n-1)}_{x,y}).
% \end{equation}


\subsubsection{Encoding and Encrypting Filters}

Due to the above method for encoding/encrypting input data,
all the values encoded/encrypted in one same ciphertext needs to be multiplied with one same element of a filter at a time.
Hence, each element $F_{i,j}$ of a filter $F$ should be duplicated for $n\cdot\tilde{\beta}_0^2$ times 
and then encoded/encrypted into a ciphertext denoted as $\hat{F}_{i,j}$. 


% \paragraph{Optimization}

% When $n\cdot\tilde{\beta}_0^2$ is much smaller than $s$ (i.e., the number of slots contained in a ciphertext),
% multiple ciphertexts of different channels can be combined into a ciphertext,
% and the corresponding ciphertexts for filter matrix elements 
% should be combined accordingly.
% %
% Specifically, 
% assuming $n\cdot\tilde{\beta}_0^2\cdot\alpha\leq\frac{s}{m}$ for certain factor $m$ of both $\alpha$ and $s$,
% for each $k\in\{0,\cdots,m-1\}$ and each $u,v\in\{0,\cdots,\tilde{\gamma}_0-1\}$,
% $\vec{I}_{k\cdot m,u,v},\vec{I}_{k\cdot m+1,u,v},\cdots,\vec{I}_{k\cdot m + \frac{s}{m}-1,u,v}$
% can be concatenated into a new vector $\vec{I}_{k,u,v}$ which 
% is then encrypted to a new ciphertext $\vec{C}_{k,u,v}$;
% correspondingly, for each convolutional layer $l$ and each pair $(u,v)$ where $u,v\in\{0,\cdots,\beta_l-1\}$,
% the element with the same index $(u,v)$ in each of filter matrices of multiple channels 
% are each duplicated for $n\cdot\tilde{\beta}_0^2\cdot m$ times and then concatenated to form a vector,
% which is then encrypted to a ciphertext.

% If $n\cdot\tilde{\beta}_0^2\cdot\alpha < s$ and $n\cdot\tilde{\beta}_0^2\cdot\alpha$ is a factor of $s$,
% the afore-mentioned combined ciphertext with $m=\alpha$
% can be further duplicated for $m'=\frac{s}{n\cdot\tilde{\beta}_0^2\cdot\alpha}$ times;
% accordingly, 
% can be further optimized by duplicating the above-mentioned ciphertext for multiple times; 
% accordingly, the elements from multiple filter matrices that need to be multiplied with the ciphertexts should be combined. 

% In the following, however, 
% we do not incorporate the optimizations for clarity and simplicity of presentation.  



% When the slots cannot be used completely, 
% multiple channels can be combined; hence,
% elements from multiple filters corresponding to the channels can be combined together.


\subsection{Propagation through Convolutional Layer $l$}

% To facilitate the description, 
% we first generalize the definitions of 
% %$\tilde{\delta}_0$, 
% $\tilde{\gamma}_0$ 
% % and $\tilde{\beta}_0$ 
% to those of
% % $\tilde{\delta}_l$, 
% $\tilde{\gamma}_l$ 
% % and $\tilde{\beta}_l$ 
% for $l=0,\cdots,c-1$, 
% as follows:
% % \begin{equation}\label{eq:tilde-delta-l}
% %     \tilde{\delta}_l = \prod_{i=l}^{c-1}\delta_i,
% % \end{equation}
% %
% \begin{equation}
%     \tilde{\gamma}_l = 1 + \sum_{i=l}^{c-1}(\gamma_i-1)\prod_{j=l}^{i-1}\delta_j,
% \end{equation}
% %
% % and 
% % \begin{equation}
% %     \tilde{\beta}_l = 1 + \lfloor\frac{\beta_l-\tilde{\gamma}_l}{\tilde{\delta}_l}\rfloor.
% % \end{equation}
% which is equivalent to 
% \begin{equation}
%     \tilde{\gamma}_l = \gamma_l + (\tilde{\gamma}_{l+1}-1)\cdot \delta_l.
% \end{equation}

With the above method for encoding and encryption,
each propagation layer $l$ has $\tilde{\gamma}_l^2$ input ciphertexts for each channel;
they can be treated as elements of an encrypted input matrix of dimensions $\tilde{\gamma}_l\times\tilde{\gamma}_l$.
We denote these input ciphertexts as $\hat{C}^{(l)}_{i,u,v}$ for 
every channel $i\in\{0,\cdots,\alpha_{l}-1\}$ and every pair $(u,v)\in\{0,\cdots,\tilde{\gamma}_l-1\}^2$.
Convolutional operations are then performed between 
these input ciphertexts and the encrypted elements of the filters.
The encrypted elements of the filters are denoted as 
$\hat{F}^{(l,k)}_{i,x,y}$ for 
every channel $i$,
every filter with index $k\in\{0,\cdots,\epsilon_l-1\}$ of the channel, 
and every element index $(x,y)\in\{0,\cdots,\gamma_l-1\}^2$ of a filter matrix.
Then, the activation function, which is a square function in this paper, 
is applied at each of the resulting neurons. 
Finally, propagating through the layer results in the following outputs:
$\hat{C}^{(l+1)}_{k,u,v}$ for every output channel $k\in\{0,\cdots,\epsilon_l-1\}$
and every pair $(u,v)\in\{0,\cdots,\tilde{\gamma}_{l+1}-1\}^2$.
Note that, the outputs become the inputs of the next layer;
when $l=c=1$, each output channel has only one output ciphertext, 
i.e., $\tilde{\gamma}_{c}=1$.
The procedure is formally presented in Algorithm~\ref{alg:fwd-conv-layer}.


% Right before the propagation through a convolutional layer $l$,
% for each channel $i$, 
% each input matrix should have already encrypted into $\tilde{\gamma}_l^2$ ciphertexts,
% each of which can be indexed by a unique $(u,v)\in\{0,\cdots,\tilde{\gamma}_l-1\}^2$;
% we denote the afore-mentioned input matrix as $\vec{I}^{(l)}_{i,u,v}$ and 
% the ciphertext as $\vec{C}^{(l)}_{i,u,v}$. 
% %
% For the same channel $i$,
% each element with index $(u,v)\in\{0,\cdots,\gamma_l-1\}^2$ 
% of each filter matrix with index $k\in\{0,\cdots,f_l-1\}$ 
% is encrypted to ciphertext $\hat{F}^{(l,k)}_{i,u,v}$.

% While propagating through the layer,

% Algorithm~\ref{alg:fwd-conv-layer} formally presents how the forward propagation is conducted
% through a convolutional layer $l$.

\begin{algorithm}[htb]
\SetAlgoLined
\caption{Propagation through Conv. Layer $l$}
\label{alg:fwd-conv-layer}
\scriptsize

% \begin{algorithmic}[1]

\For{$k\in\{0,\cdots,\epsilon_l-1\}$}{ 
        \For{$(u,~v)\in\{0,\cdots,\tilde{\gamma}_{l+1}-1\}^2$}{
            % \For{$v\in\{0,\cdots,\tilde{\gamma}_{l+1}-1\}$} 
                $\hat{C}^{(l+1)}_{k,u,v}\leftarrow 0$; 
                \Comment{initialize each output}\;
                $(u',~v')\leftarrow (\delta_l\cdot u,~\delta_l\cdot v)$\;
                % \State $v'\leftarrow \delta_l\cdot v$
                \For{$(x,~y)\in\{0,\cdots,\gamma_l-1\}^2$}{
                    % \For{$y\in\{0,\cdots,\gamma_l-1\}$}
                        \For{$i\in\{0,\cdots,\alpha_l-1\}$}{ 
                            $\hat{C}^{(l+1)}_{k,u,v}\oplus = \hat{C}^{(l)}_{i,u'+x,v'+y}\otimes\hat{F}^{(l,k)}_{i,x,y}$;
                        }
                        % \EndFor
                    % \EndFor
                }
                % \EndFor 
                $\hat{C}^{(l+1)}_{k,u,v}\leftarrow \hat{C}^{(l+1)}_{k,u,v}\otimes\hat{C}^{(l+1)}_{k,u,v}$; 
                \Comment{activation}
            % \EndFor
        }
        % \EndFor
}
% \EndFor

% \end{algorithmic}
\end{algorithm}




% \subsection{Propagation through Pooling Layer $l$}

% (skip for now)

\subsection{Propagation through Fully-connected Layer $l$}

% We use the following notations to facilitate our presentation. 
Recall that the input to layer $l$ is 
the intermediate results of processing $n$ original inputs,
and the processing for these $n$ inputs are in parallel independently.
%
% We use $\iota_l$ to denote the number of values in the input to layer $l$ that are from each of the $n$ original inputs;
% hence, totally there are $\iota_l\cdot n$ distinct input values encoded/encrypted in the input to layer $l$.
%
Due to our method for encoding (as in Section~\ref{sec:encoding}),
the input values that are of the same offset but from $n$ different original inputs 
are encoded consecutively (as in Eq.~(\ref{eq:initial-input-format-2})),
we call such sequence of $n$ values as a {\em parallel input set (pi-set)}. 
%Obviously, each set encodes $n$ values. 
We use $\iota_l$ to denote the number of pi-sets encoded/encrypted into the input of layer $l$;
thus, the input of layer $l$ encodes/encrypts totally $\iota_l\cdot n$ values. 
% Hence, the input to layer $l$ encodes/encrypts of $\iota_l$ sets (i.e., totally $\iota_l\cdot n$) of distinct input values.
%
We further use $\iota'_l$ to denote the number of ciphertexts in the input to layer $l$, and denote
the ciphertexts as $\hat{C}^{(l)}_0,\cdots,\hat{C}^{(l)}_{\iota'_l-1}$.
Our design evenly distributes the $\iota_l$ pi-sets to the $\iota'_l$ ciphertexts; thus, 
each ciphertext encodes/encrypts $\iota''_l=\frac{\iota_l}{\iota'_l}$ pi-sets.
We also assume $\iota''_l$ is an integer for the convenience of presentation. 

The input to layer $l$ has two types.
% \begin{itemize}
%     \item 
    Type I (ciphertext input without replication):
    % For this type, 
    % such as the resulting ciphertexts from the afore-discussed convolutional layers, 
    each ciphertext encodes/encrypts multiple pi-sets in the format similar to 
    Eq.~(\ref{eq:initial-input-format-1}) and (\ref{eq:initial-input-format-2}), 
    in which the pi-sets are not replicated.
    % \item 
    Type II (ciphertext input with replication):
    each ciphertext contains one pi-set which is replicated for multiple times. 
% \end{itemize}
Next, we present the algorithms for propagating through layer $l$ with each type of input.



\subsubsection{Propagation with Type I Input}
\label{sec:forward-full-1}

%forward propagation needs rotation; but backward does not

% Generally, the convolutional layers result in a setting where 
% each input ciphertext contains multiple sets of input elements. 

% Suppose all the $\iota_l$ sets of input elements are stored in $\iota'_l$ ciphtertexts,
% which are denoted as $\tilde{C}^{(l)}_0,\cdots,\tilde{C}^{(l)}_{\iota'_l-1}$,
% and each of such ciphertext contains $\iota''_l$ sets of input elements; 
% hence, $\iota_l=\iota'_l\cdot\iota''_l$.
% Note that, the size of each set is $n$ as there are $n$ sets of learning data processed per epoch.

In this case, each input ciphertext $\hat{C}^{(l)}_j$ for $j\in\{0,\cdots,\iota'_l-1\}$
encodes and encrypts $\iota''_l$ pi-sets.
%
As presented in Section~\ref{subsec:cnn-model},
the weight matrix for the layer is $M^{(l)}$ with dimensions $\iota_l\times o_l$;
let us denote the elements of $M^{(l)}$ as 
$M^{(l)}_{u,v}$ where $u\in\{0,\cdots,o_l-1\}$ and $v\in\{0,\cdots,\iota_l-1\}$.  
%
To facilitate efficient forward propagation through this layer,
the elements of $M^{(l)}$ are encoded and encrypted to $o_l\cdot\iota'_l$ ciphertexts,
denoted as $\hat{M}^{(l)}_{i,j}$ for every $i\in\{0,\cdots,o_l-1\}$ and every $j\in\{0,\cdots,\iota'_l-1\}$.
Here, each $\hat{M}^{(l)}_{i,j}$ encrypts the following vector
\begin{equation}\scriptsize
    (\vec{M}^{(l)}_{i,j\cdot\iota''_l}, \cdots, \vec{M}^{(l)}_{i,(j+1)\cdot\iota''_l-1}),
\end{equation}
where for each $w\in\{j\cdot\iota''_l,\cdots,(j+1)\cdot\iota''_l-1\}$,
$\vec{M}^{(l)}_{i,w}$ stands for a sequence of $n$ duplicated values of ${M}^{(l)}_{i,w}$; i.e., 
\begin{equation}\scriptsize
    \vec{M}^{(l)}_{i,w} = ({M}^{(l)}_{i,w},\cdots,{M}^{(l)}_{i,w}). 
\end{equation}
% $M_l[i][j\cdot\iota''_l],\cdots,M_l[i][(j+1)\cdot\iota''_l-1]$.

Algorithm~\ref{alg:fwd-full-layer-I} formally presents the forward propagation.
%
% To understand this algorithm,
% let us consider how the $i$=th output values for all the $n$ original inputs are computed.
% We denote the 
% If there is no encryption, this output value should be computed as 
% \begin{equation}
%     \sum_{j=0}^{\iota_l-1} M^{(l)}_{i,j}\cdot 
% \end{equation}
%
% Specifically, each output ciphertext $\hat{C}^{(l+1)}_i$ for 
% $i\in\{0,\cdots,o_l-1\}$ is computed as follows.
% First, with the loop on lines 3-5, 
%
% is conducted through a type-I fully-connected layer $l$.
This results in $o_l$ ciphertexts, each encoding/encrypting 
$\frac{\cal S}{n}$ replicas of a set of $n$ output values.
Note that, if the output is used as the input of the next layer,
it becomes a type II input. 


\begin{algorithm}[htb]
\SetAlgoLined
\caption{Propagation through Fully-connected Layer $l$ (with Type I Input)}
\label{alg:fwd-full-layer-I}
\scriptsize

% \begin{algorithmic}[1]

\For{$i\in\{0,\cdots,o_l-1\}$}{
    $\hat{C}^{(l+1)}_i\leftarrow 0$; \Comment{initialize each output ciphertext}\;
    \For{$j\in\{0,\cdots,\iota'_l-1\}$}{
        $\hat{C}^{(l+1)}_i \oplus = \hat{C}^{(l)}_{j}\otimes\hat{M}^{(l)}_{i,j}$;
    }
    \For{$j\in\{1,\cdots,\log(\frac{\cal S}{n})\}$}{
        $\hat{C}^{(l+1)}_i \oplus= Rot(\hat{C}^{(l+1)}_i,j\cdot n)$;
    }
    $\hat{C}^{(l+1)}_i\leftarrow \hat{C}^{(l+1)}_i\otimes\hat{C}^{(l+1)}_i$; 
    \Comment{activation}
}
    % \State $\tilde{C}^{(l+1)}_i\leftarrow 0$ \Comment{each output element $i$}
    % \For{$j\in\{0,\cdots,\iota'_l-1\}$} 
    %     \State $\tilde{C}^{(l+1)}_i += \tilde{C}^{(l)}_{j}\bigodot\tilde{M}^{(l)}_{i,j}$
    % \EndFor
    % \For{$j\in\{1,\cdots,\log(\frac{s}{n})\}$}
    %     \State $\tilde{C}^{(l+1)}_i += Rotate(\tilde{C}^{(l+1)}_i,j\cdot n)$
    % \EndFor
% \EndFor

% \end{algorithmic}
\end{algorithm}



\subsubsection{Propagation with Type II Input}

%forward propagation or backward propagation does not need rotation

In this case,
the input has $\iota'_l=\iota_l$ ciphertexts
each encrypting $\frac{\cal S}{n}$ replicas of only one input set (i.e., $n$ input values from $n$ original inputs).
%
To facilitate the propagation,
the elements of weight matrix $M^{(l)}$ are encrypted to 
$\iota_l\cdot\lceil\frac{o_l\cdot n}{\cal S}\rceil$ ciphtertexts,
denoted as $\hat{M}^{(l)}_{i,j}$ for 
$i\in\{0,\cdots,\iota_l-1\}$ and $j\in\{0,\cdots,\lceil\frac{o_l\cdot n}{\cal S}\rceil-1\}$,
where each $\hat{M}^{(l)}_{i,j}$ encodes and encrypts the following vector
\begin{equation}\scriptsize
    (\vec{M}^{(l)}_{j\cdot\frac{\cal S}{n},i},\cdots,\vec{M}^{(l)}_{\min\{(j+1)\cdot\frac{\cal S}{n},o_l\}-1,i}),
\end{equation}
where for each $w\in\{j\cdot\frac{\cal S}{n},\cdots,\min\{(j+1)\cdot\frac{\cal S}{n},o_l\}-1\}$, 
$\vec{M}^{(l)}_{w,i}$ stands for a sequence of $n$ duplicated values of ${M}^{(l)}_{w,i}$.

% weights
% $M_l[j\cdot\frac{s}{n}][i],\cdots,M_l[\min\{j\cdot\frac{s}{n},o_l\}-1][i]$.

Algorithm~\ref{alg:fwd-full-layer-II} formally presents how the forward propagation
is conducted through a type-II fully-connected layer $l$.
This results in $\lceil\frac{o_l\cdot n}{\cal S}\rceil$ ciphertexts
each encoding/encrypting $\frac{\cal S}{n}$ pi-sets.
Note that, if the output is used as the input for the next layer,
it becomes a Type I input. 

\begin{algorithm}[htb]
\SetAlgoLined
\caption{Propagation through Fully-connected Layer $l$ (with Type II Input)}
\label{alg:fwd-full-layer-II}
\scriptsize

\For{$i\in\{0,\cdots,\lceil\frac{o_l\cdot n}{\cal S}\rceil-1\}$}{
    $\hat{C}^{(l+1)}_i\leftarrow 0$; \Comment{each output element $i$}\;
    \For{$j\in\{0,\cdots,\iota_l-1\}$}{
        $\hat{C}^{(l+1)}_i \oplus= \hat{C}^{(l)}_{j}\otimes\hat{M}^{(l)}_{i,j}$
    }
    $\hat{C}^{(l+1)}_i\leftarrow \hat{C}^{(l+1)}_i\otimes\hat{C}^{(l+1)}_i$; 
    \Comment{activation}
}

\end{algorithm}


\begin{algorithm}[htb]
\SetAlgoLined
\caption{Backward Propagation through Fully-connected Layer $l$ (with Type II Input)}
\label{alg:bwd-full-layer-II}
\scriptsize
\For{$j\in\{0,\cdots,\lceil\frac{o_l\cdot n}{\cal S}\rceil-1\}$}{
    $\tilde{C}^{(l+1)}_j \leftarrow 2\otimes\tilde{C}^{(l+1)}_{j}$
    \Comment{activation derivation}
}
\For{$i\in\{0,\cdots,\iota_l-1\}$}{
    $\tilde{C}^{l}_i\leftarrow 0$; \Comment{each input element $i$}\;
    \For{$j\in\{0,\cdots,\lceil\frac{o_l\cdot n}{\cal S}\rceil-1\}$}{
        $\tilde{C}^{(l)}_i \oplus= \tilde{C}^{(l+1)}_{j}\otimes\hat{M}^{(l)}_{j,i}$
    }
    \For{$j\in\{1,\cdots,\log(\frac{\cal S}{n})\}$}{
        $\tilde{C}^{(l)}_i \oplus= Rot(\tilde{C}^{(l)}_i,j\cdot n)$;
    }
}

\end{algorithm}


\begin{algorithm}[htb]
\SetAlgoLined
\caption{Backward Propagation through Fully-connected Layer $l$ (with Type I Input)}
\label{alg:bwd-full-layer-I}
\scriptsize
\For{$j\in\{0,\cdots,o_l-1\}$}{
    $\tilde{C}^{(l+1)}_j \leftarrow 2\otimes\tilde{C}^{(l+1)}_{j}$
    \Comment{activation derivation}
}
\For{$i\in\{0,\cdots,\iota'_l-1\}$}{
    $\tilde{C}^{(l)}_i\leftarrow 0$; \Comment{each input element $i$}\;
    \For{$j\in\{0,\cdots,o_l-1\}$}{
        $\tilde{C}^{(l)}_i \oplus= \tilde{C}^{(l+1)}_{j}\otimes\hat{M}^{(l)}_{j,i}$
    }
}

\end{algorithm}

\begin{algorithm}[htb]
\SetAlgoLined
\caption{Compute Rotation directions and steps}
\label{alg:bwd-cpt-rotation}
\scriptsize
$\vec{R}\leftarrow 1$;
\Comment{initialize output}\;
\For{$i\in\{\lceil\log n\rceil,\cdots,0\}$}{
    \If{$p\geq 2^i$}{
        $p -= 2^i$;
        $\vec{R}_i = -1$\;
    }
}

\end{algorithm}


\begin{algorithm}[htb]
\SetAlgoLined
\caption{Updating Weight Gradients through Fully-connected Layer $l$}
\label{alg:bwd-weights-full-layer}
\scriptsize
\For{$j\in\{0,\cdots,o'_l-1\}$}{ \Comment{$o'_l=o_l$ for type I and $o'_l=\lceil\frac{o_l\cdot n}{\cal S}\rceil-1$ for type II}\;
    \For{$i\in\{0,\cdots,\iota'_l-1\}$}{
        $\tilde{M}^{(l)}_{j,i} = \tilde{C}^{(l+1)}_{j}\otimes\hat{C}^{(l)}_{i}$;
    }
}
\For{$j\in\{0,\cdots,o'_l-1\}$}{ 
    \For{$i\in\{0,\cdots,\iota'_l-1\}$}{
        \Comment{sum up gradients from $n$ parallel images to position $p$ for $\tilde{M}^{(l)}_{j,i}$}\;
        $p \leftarrow (j\cdot\iota'_l+i)\%n$\;
        $\vec{R} \leftarrow computeRotations(p, n)$; 
        \Comment{compute the rotate directions and steps to sum up gradients}\;
        \For{$k\in\{0,\cdots,\lceil\log n\rceil\}$}{
            $\tilde{M}^{(l)}_{j,i} \oplus= Rot(\tilde{M}^{(l)}_{j,i}, 2^k\cdot\vec{R}_k)$;
        }
        $\hat{M}^{(l)}_{j,i} \oplus= \tilde{M}^{(l)}_{j,i}$;
        \Comment{update weight with gradients}
    }
}
\end{algorithm}

\begin{algorithm}[htb]
\SetAlgoLined
\caption{Remove accumulated noise of Weights in Fully-connected Layer $l$}
\label{alg:bwd-weights-TEE-full-layer}
\scriptsize
\For{$j\in\{0,\cdots,o'_l-1\}$}{ 
    \For{$i\in\{0,\cdots,\iota'_l-1\}$}{
        \Comment{pack weights $\hat{M}^{(l)}_{j,i}$ together}\;
        $(p,~k)\leftarrow ((j\cdot\iota'_l+i)\%n,~(j\cdot\iota'_l+i)/n)$\;
        $\vec{U} \leftarrow [0,\cdots,1,\cdots,0,\cdots,1,\cdots]$;
        \Comment{for position $\{p,p+n,p+2n,\cdots,p+\lfloor\frac{{\cal S} -p}{n}\rfloor\cdot n\}$, $\vec{U}$ has value 1, otherwise 0}\;
        \If{not visited $k$}{
            $\hat{PM}^{(l)}_k\leftarrow 0$;
            \Comment{initialize each output}\;
        }
        $\hat{PM}^{(l)}_k \oplus= \hat{M}^{(l)}_{j,i}\otimes\vec{U}$; 
    }
}
\For{$k\in\{0,\cdots,\lceil\frac{o'_l\cdot\iota'_l}{n}\rceil-1\}$}{
    \Comment{decrypt, decode, re-encode and re-encrypt the packed weights in TEE}\;
    $\vec{pt}\leftarrow Dec_{sk}(\hat{PM}^{(l)}_k)$;
    $\hat{PM}^{(l)}_k \leftarrow Enc_{pk}(\vec{pt})$;
}
\For{$j\in\{0,\cdots,o'_l-1\}$}{ 
    \For{$i\in\{0,\cdots,\iota'_l-1\}$}{
        \Comment{unpack weights $\hat{PM}^{(l)}_k$ and recover $\hat{M}^{(l)}_{j,i}$}\;
        $(p,~k)\leftarrow ((j\cdot\iota'_l+i)\%n,~(j\cdot\iota'_l+i)/n)$\;
        $\vec{U} \leftarrow [0,\cdots,1,\cdots,0,\cdots,1,\cdots]$;
        \Comment{for position $\{p,p+n,p+2n,\cdots,p+\lfloor\frac{{\cal S} -p}{n}\rfloor\cdot n\}$, $\vec{U}$ has value 1, otherwise 0}\;
        $\hat{M}^{(l)}_{j,i} \leftarrow \hat{PM}^{(l)}_k\otimes\vec{U}$\; 
        $\vec{R} \leftarrow computeRotations(p, n)$; 
        \Comment{compute the rotate directions and steps to spread gradients}\;
        \For{$t\in\{0,\cdots,\lceil\log n\rceil\}$}{
            $\hat{M}^{(l)}_{j,i} \oplus= Rot(\hat{M}^{(l)}_{j,i}, -2^t\cdot\vec{R}_t)$;
        }
    }
}
\end{algorithm}

\begin{algorithm}[htb]
\SetAlgoLined
\caption{Backward Propagation through Conv. Layer $l$}
\label{alg:bwd-conv-layer}
\scriptsize
\For{$i\in\{0,\cdots,\alpha_l-1\}$}{ 
    \For{$(u,~v)\in\{0,\cdots,\tilde{\gamma}_{l+1}-1\}^2$}{
        $(u',~v')\leftarrow (\delta_l\cdot u,~\delta_l\cdot v)$\;
        \For{$(x,~y)\in\{0,\cdots,\gamma_l-1\}^2$}{
            \For{$k\in\{0,\cdots,\epsilon_l-1\}$}{ 
                \If{not visited $(u'+x, v'+y)$}{
                $\tilde{C}^{(l)}_{i,u'+x,v'+y}\leftarrow 0$;
                \Comment{initialize each output}\;
                }
                $\tilde{C}^{(l)}_{i,u'+x,v'+y}\oplus = \tilde{C}^{(l+1)}_{k,u,v}\otimes\hat{F}^{(l,k)}_{i,x,y}$;
            }
        }
        
    }
}

\end{algorithm}


\begin{algorithm}[htb]
\SetAlgoLined
\caption{Updating Kernal Gradients through Conv. Layer $l$}
\label{alg:bwd-kernals-conv-layer}
\scriptsize
\For{$k\in\{0,\cdots,\epsilon_l-1\}$}{ 
    \For{$i\in\{0,\cdots,\alpha_l-1\}$}{
        \For{$(x,~y)\in\{0,\cdots,\gamma_l-1\}^2$}{
            $\tilde{F}^{(l,k)}_{i,x,y}\leftarrow 0$;
            \Comment{initialize each output}\;
            \For{$(u,~v)\in\{0,\cdots,\tilde{\gamma}_{l+1}-1\}^2$}{
                $(u',~v')\leftarrow (\delta_l\cdot u,~\delta_l\cdot v)$\;
                $\tilde{F}^{(l,k)}_{i,x,y}\oplus = \hat{C}^{(l)}_{i,u'+x,v'+y}\otimes\tilde{C}^{(l+1)}_{k,u,v}$;
            }
            $p \leftarrow (k\cdot\alpha\gamma_l^2+i\cdot\gamma_l^2+x\cdot\gamma_l+y)\%n$\;
            $\vec{R} \leftarrow computeRotations(p, n)$; 
            \Comment{compute the rotate directions and steps to sum up gradients}\;
            \For{$t\in\{0,\cdots,\lceil\log n\rceil\}$}{
            \Comment{sum up gradients from $n$ parallel images}\;
                $\tilde{F}^{(l,k)}_{i,x,y} \oplus= Rot(\tilde{F}^{(l,k)}_{i,x,y}, 2^t\cdot\vec{R}_t)$;
            }
            $\hat{F}^{(l,k)}_{i,x,y} \oplus= \tilde{F}^{(l,k)}_{i,x,y}$;
            \Comment{update kernal with gradients}
        }
    }
}

\end{algorithm}


\begin{algorithm}[htb]
\SetAlgoLined
\caption{Remove accumulated noise of Kernals in Conv. Layer $l$}
\label{alg:bwd-kernals-TEE-conv-layer}
\scriptsize
\For{$k\in\{0,\cdots,\epsilon_l-1\}$}{ 
    \For{$i\in\{0,\cdots,\alpha_l-1\}$}{
        \For{$(x,~y)\in\{0,\cdots,\gamma_l-1\}^2$}{
            \Comment{pack kernals $\hat{F}^{(l,k)}_{i,x,y}$ together}\;
            $idx \leftarrow k\cdot\alpha\gamma_l^2+i\cdot\gamma_l^2+x\cdot\gamma_l+y$\;
            $(p, t) \leftarrow (idx\%n, idx/n)$\;
            $\vec{U} \leftarrow [0,\cdots,1,\cdots,0,\cdots,1,\cdots]$;
            \Comment{for position $\{p,p+n,p+2n,\cdots,p+\lfloor\frac{{\cal S} -p}{n}\rfloor\cdot n\}$, $\vec{U}$ has value 1, otherwise 0}\;
            \If{not visited $t$}{
                $\hat{PF}^{(l)}_t\leftarrow 0$;
                \Comment{initialize each output}\;
            }
            $\hat{PF}^{(l)}_t\oplus=\hat{F}^{(l,k)}_{i,x,y}\otimes\vec{U}$\;
        }
    }
}
\For{$k\in\{0,\cdots,\lceil\frac{\epsilon_l\cdot\alpha_l\cdot\gamma_l^2}{n}\rceil-1\}$}{
    \Comment{decrypt, decode, re-encode and re-encrypt the packed weights in TEE}\;
    $\vec{pt}\leftarrow Dec_{sk}(\hat{PF}^{(l)}_k)$;
    $\hat{PF}^{(l)}_k \leftarrow Enc_{pk}(\vec{pt})$;
}
\For{$k\in\{0,\cdots,\epsilon_l-1\}$}{ 
    \For{$i\in\{0,\cdots,\alpha_l-1\}$}{
        \For{$(x,~y)\in\{0,\cdots,\gamma_l-1\}^2$}{
            \Comment{unpack weights $\hat{PF}^{(l)}_t$ and recover $\hat{F}^{(l,k)}_{i,x,y}$}\;
            $idx \leftarrow k\cdot\alpha\gamma_l^2+i\cdot\gamma_l^2+x\cdot\gamma_l+y$\;
            $(p, t) \leftarrow (idx\%n, idx/n)$\;
            $\vec{U} \leftarrow [0,\cdots,1,\cdots,0,\cdots,1,\cdots]$\;
            \Comment{for position $\{p,p+n,p+2n,\cdots,p+\lfloor\frac{{\cal S} -p}{n}\rfloor\cdot n\}$, $\vec{U}$ has value 1, otherwise 0}\;
            $\hat{F}^{(l,k)}_{i,x,y}\leftarrow\hat{PF}^{(l)}_t\otimes\vec{U}$\;
            $\vec{R} \leftarrow computeRotations(p, n)$; 
            \Comment{compute the rotate directions and steps to spread gradients}\;
            \For{$s\in\{0,\cdots,\lceil\log n\rceil\}$}{
                $\hat{F}^{(l,k)}_{i,x,y} \oplus= Rot(\hat{F}^{(l,k)}_{i,x,y}, -2^s\cdot\vec{R}_s)$;
            }
        }
    }
}
\end{algorithm}

\subsubsection{Further Optimizations}

With the above algorithms,
each initial input ciphertext encodes/encrypts $n\cdot\tilde{\beta}_0^2$ input values.
If $n\cdot\tilde{\beta}_0^2$ is much less than ${\cal S}$ (i.e., 
the number of slots in a ciphertext),
the slots will not be effectively utilized and 
the system efficiency will be degraded.
Hence, we propose cross-channel and cross-filter packing.
% in this section.
%
% When the number of available data sets $n$ is small or the slots number $s$ is much larger than $n\cdot\tilde{\beta}_0^2$, in order to fully utilize the slots in a ciphertext, we propose two ways to optimize the packing methods of the convolutional layer from the basic scheme. 
%
Specifically, 
letting $r$ be the largest power of $2$ which is no greater than $\frac{\cal S}{n\cdot\tilde{\beta}_0^2}$, 
the inputs from $r$ channels can be encoded together such that more input values can be processed in parallel, 
or each ciphertext can encode/encrypt $r$ replicas of the original $n\cdot\tilde{\beta}_0^2$ values such that
the same input can be processed with multiple filters in parallel. 
Such changes, however, also demand according changes to the procedure of 
propagation through each convolutional layer.
Due to space limit, we skip the details
% ed description of these optimizations
though we have incorporated them in our prototype system. 
%In this section, we elaborate on these optimizations. 




\begin{figure*}[htb]
    \centering
    \caption{An Example.}
    % of Proposed Solution. Each matrix represents the original data and each vector represents one ciphertext with multiple data packed.}
    \label{fig:example}
    \includegraphics[width=\textwidth]{example.drawio.pdf}
\end{figure*}

\subsection{An Example}

Figure~\ref{fig:example} illustrates a simple example,
where our proposed scheme is applied to a CNN model of $2$ CLs and $2$ FLs and 
activation function is not considered.
Two $8\times 8$ input matrices, 
labelled as $I_1$ and $I_2$, 
are processed in parallel. 
Thus, $16$ ciphertexts are constructed to encode/encrypt the values of the input matrices.
Each ciphertext encodes/encrypts $8$ input values,
represented as $4$ cells.
Each cell contains $2$ values from the $2$ input matrices respectively; recall that
such a cell is called pi-set in the description of our scheme. 

CL1 has two $2\times2$ filter matrices, 
labelled as $f_1$ and $f_2$, each has one channel. 
%
CL2 also has two $2\times2$ filters, 
labelled as $c_1$ and $c_2$, each belonging to a separated channel. 
%
Each filter is encrypted to $4$ ciphertexts, 
and each ciphtertext contains $8$ replicated elements to 
match the ciphertexts for input values.
%
The output from the two CLs is one single ciphertext,
which is a Type I input to layer FL1. 

FL1 has $4$ input and $2$ output neurons as inferred from its $4\times2$ weight matrix.
The elements of the matrix is encrypted to $2$ ciphertexts 
corresponding to the $2$ output neurons respectively.
Now, the outputs should be computed as the dot-products of 
the vector encoded/encrypted in the input ciphertext and 
each of the vectors encoded/encrypted in the weight-matrix's ciphertexts. 
This is accomplished according to Algorithm~\ref{alg:fwd-full-layer-I},
and the call-out on the left-hand side illustrates 
the steps for computing the first of the outputs: 
% \begin{itemize}
%     \item 
    
{\underline{First}}, the input ciphertext that encrypts $(20,40,28,56,84,168,92,184)$ HE-multiplies with
    the first ciphertext of the weight matrix, which encrypts $((1,1,0,0,0,0,1,1)$;
    this results in the ciphertext that encrypts $(20,40,0,0,0,0,92,184)$.
    
    % \item 
{\underline{Second}}, the ciphertext for $(20,40,0,0,0,0,92,184)$ HE-adds 
    a copy of itself which but also rotates (to left) for one cell,
    and this results in a ciphertext for $(20,40,0,0,92,184,112,224)$.
    
    % \item
{\underline{Third}}, the ciphertext for HE-adds a copy of itself which also rotates (to left) for $2$ cells,
    and this results in a ciphertext for $(112,224,112,224,112,224,112,224)$.

% \end{itemize}
The result of the above steps becomes a type II input for the next layer, FL2.
%
For FL2, the weights connected to the same input neuron are packed into one ciphertext;
hence, there are $2$ ciphertexts for the weights.
Each of the $2$ ciphertexts multiplies with the corresponding input ciphertext,
and resulting $2$ product-ciphertexts are added up to get the final result,
which encrypts $(36,72,0,0,0,0,76,152)$.


% For filter $f_1$ and $f_2$, each is encrypted into 4 ciphertexts.
% The outputs of CL1 has 2 channels and each channel contains 4 ciphertexts.
% There are 1 filter in CL2 and contains 2 channels $c_1$ and $c_2$, each channel is of dimension $2\times2$.
% Same as filters in CL1, each value inside filter is duplicated and encrypted into one ciphertext.
% After 2 CLs, the outputs are packed into one ciphertext.
% The weight matrix $w_1$ in FL1 and $w_2$ in FL2 has dimension $4\times2$ and $2\times4$ respectively.
% $w_1$ has all weights connected to the same output neuron packed together. 
% Then it requires 2 ciphertext to pack $w_1$.
% In order to get the correct results of FL1, we need to rotate the results after the input and packed weight multiplication.
% The detailed steps for the rotation to get the FL1 output
% (i.e., $(76,152,76,152,76,152,76,152)$) is also described in figure~\ref{fig:example}.
% In FL2, the weights connected to the same input neuron are packed into one ciphertext.
% Then $w_2$ is packed into 2 ciphertexts.
